Transfer Learning between Motor Imagery Datasets using Deep Learning -- Validation of Framework and Comparison of Datasets

We present a simple deep learning-based framework commonly used in computer vision and demonstrate its effectiveness for cross-dataset transfer learning in mental imagery decoding tasks that are common in the field of Brain-Computer Interfaces (BCI). We investigate, on a large selection of 12 motor-imagery datasets, which ones are well suited for transfer, both as donors and as receivers. Challenges. Deep learning models typically require long training times and are data-hungry, which impedes their use for BCI systems that have to minimize the recording time for (training) examples and are subject to constraints induced by experiments involving human subjects. A solution to both issues is transfer learning, but it comes with its own challenge, i.e., substantial data distribution shifts between datasets, subjects and even between subsequent sessions of the same subject. Approach. For every pair of pre-training (donor) and test (receiver) dataset, we first train a model on the donor before training merely an additional new linear classification layer based on a few receiver trials. Performance of this transfer approach is then tested on other trials of the receiver dataset. Significance. First, we lower the threshold to use transfer learning between motor imagery datasets: the overall framework is extremely simple and nevertheless obtains decent classification scores. Second, we demonstrate that deep learning models are a good option for motor imagery cross-dataset transfer both for the reasons outlined in the first point and because the framework presented is viable in online scenarios. Finally, analysing which datasets are best suited for transfer learning can be used as a reference for future researchers to determine which to use for pre-training or benchmarking.

==> export/table_all.tex <==

\begin{tabular}{lm{\colwidth}m{\colwidth}m{\colwidth}m{\colwidth}m{\colwidth}m{\colwidth}m{\colwidth}m{\colwidth}m{\colwidth}m{\colwidth}m{\colwidth}m{\colwidth}m{\colwidth}m{\colwidth}m{\colwidth}m{\colwidth}m{\colwidth}m{\colwidth}m{\colwidth}m{\colwidth}m{\colwidth}m{\colwidth}m{\colwidth}m{\colwidth}m{\colwidth}m{\colwidth}m{\colwidth}m{\colwidth}m{\colwidth}m{\colwidth}m{\colwidth}m{\colwidth}m{\colwidth}m{\colwidth}m{\colwidth}m{\colwidth}m{\colwidth}m{\colwidth}m{\colwidth}m{\colwidth}m{\colwidth}m{\colwidth}m{\colwidth}m{\colwidth}m{\colwidth}m{\colwidth}m{\colwidth}m{\colwidth}}
\textbf{Test dataset} & \multicolumn{5}{l}{{\cellcolor[rgb]{.9,.9,.9}} AlexMI} & \multicolumn{6}{l}{BNCI2014001} & \multicolumn{6}{l}{{\cellcolor[rgb]{.9,.9,.9}} BNCI2015004} & \multicolumn{6}{l}{Ofner2017(I)} & \multicolumn{5}{l}{{\cellcolor[rgb]{.9,.9,.9}} PhysionetMI(I)} & \multicolumn{7}{l}{Schirrmeister2017} & \multicolumn{7}{l}{{\cellcolor[rgb]{.9,.9,.9}} Weibo2014} & \multicolumn{6}{l}{Zhou2016} \\
\textbf{Trials/class} & {\cellcolor[rgb]{.9,.9,.9}} 1 & 2 & {\cellcolor[rgb]{.9,.9,.9}} 4 & 8 & {\cellcolor[rgb]{.9,.9,.9}} 16 & 1 & {\cellcolor[rgb]{.9,.9,.9}} 2 & 4 & {\cellcolor[rgb]{.9,.9,.9}} 8 & 16 & {\cellcolor[rgb]{.9,.9,.9}} 32 & 1 & {\cellcolor[rgb]{.9,.9,.9}} 2 & 4 & {\cellcolor[rgb]{.9,.9,.9}} 8 & 16 & {\cellcolor[rgb]{.9,.9,.9}} 32 & 1 & {\cellcolor[rgb]{.9,.9,.9}} 2 & 4 & {\cellcolor[rgb]{.9,.9,.9}} 8 & 16 & {\cellcolor[rgb]{.9,.9,.9}} 32 & 1 & {\cellcolor[rgb]{.9,.9,.9}} 2 & 4 & {\cellcolor[rgb]{.9,.9,.9}} 8 & 16 & {\cellcolor[rgb]{.9,.9,.9}} 1 & 2 & {\cellcolor[rgb]{.9,.9,.9}} 4 & 8 & {\cellcolor[rgb]{.9,.9,.9}} 16 & 32 & {\cellcolor[rgb]{.9,.9,.9}} 64 & 1 & {\cellcolor[rgb]{.9,.9,.9}} 2 & 4 & {\cellcolor[rgb]{.9,.9,.9}} 8 & 16 & {\cellcolor[rgb]{.9,.9,.9}} 32 & 64 & {\cellcolor[rgb]{.9,.9,.9}} 1 & 2 & {\cellcolor[rgb]{.9,.9,.9}} 4 & 8 & {\cellcolor[rgb]{.9,.9,.9}} 16 & 32 \\
\textbf{Pretraining dataset} & {\cellcolor[rgb]{.9,.9,.9}} & & {\cellcolor[rgb]{.9,.9,.9}} & & {\cellcolor[rgb]{.9,.9,.9}} & & {\cellcolor[rgb]{.9,.9,.9}} & & {\cellcolor[rgb]{.9,.9,.9}} & & {\cellcolor[rgb]{.9,.9,.9}} & & {\cellcolor[rgb]{.9,.9,.9}} & & {\cellcolor[rgb]{.9,.9,.9}} & & {\cellcolor[rgb]{.9,.9,.9}} & & {\cellcolor[rgb]{.9,.9,.9}} & & {\cellcolor[rgb]{.9,.9,.9}} & & {\cellcolor[rgb]{.9,.9,.9}} & & {\cellcolor[rgb]{.9,.9,.9}} & & {\cellcolor[rgb]{.9,.9,.9}} & & {\cellcolor[rgb]{.9,.9,.9}} & & {\cellcolor[rgb]{.9,.9,.9}} & & {\cellcolor[rgb]{.9,.9,.9}} & & {\cellcolor[rgb]{.9,.9,.9}} & & {\cellcolor[rgb]{.9,.9,.9}} & & {\cellcolor[rgb]{.9,.9,.9}} & & {\cellcolor[rgb]{.9,.9,.9}} & & {\cellcolor[rgb]{.9,.9,.9}} & & {\cellcolor[rgb]{.9,.9,.9}} & & {\cellcolor[rgb]{.9,.9,.9}} & \\
{\cellcolor[rgb]{.9,.9,.9}} AlexMI & {\cellcolor[HTML]{9FD899}} \color[HTML]{000000} 38 & {\cellcolor[HTML]{9CD797}} \color[HTML]{000000} 39 & {\cellcolor[HTML]{9FD899}} \color[HTML]{000000} 38 & {\cellcolor[HTML]{9CD797}} \color[HTML]{000000} 39 & {\cellcolor[HTML]{8DD08A}} \color[HTML]{000000} 43 & {\cellcolor[HTML]{BEE5B8}} \color[HTML]{000000} 28 & {\cellcolor[HTML]{BBE4B4}} \color[HTML]{000000} 29 & {\cellcolor[HTML]{B5E1AE}} \color[HTML]{000000} 31 & {\cellcolor[HTML]{AFDFA8}} \color[HTML]{000000} 33 & {\cellcolor[HTML]{A3DA9D}} \color[HTML]{000000} 37 & {\cellcolor[HTML]{95D391}} \color[HTML]{000000} 41 & {\cellcolor[HTML]{D3EECD}} \color[HTML]{000000} 20 & {\cellcolor[HTML]{D1EDCB}} \color[HTML]{000000} 21 & {\cellcolor[HTML]{D1EDCB}} \color[HTML]{000000} 21 & {\cellcolor[HTML]{CEECC8}} \color[HTML]{000000} 22 & {\cellcolor[HTML]{CCEBC6}} \color[HTML]{000000} 23 & {\cellcolor[HTML]{CAEAC3}} \color[HTML]{000000} 24 & {\cellcolor[HTML]{E2F4DD}} \color[HTML]{000000} 14 & {\cellcolor[HTML]{DFF3DA}} \color[HTML]{000000} 15 & {\cellcolor[HTML]{DFF3DA}} \color[HTML]{000000} 15 & {\cellcolor[HTML]{DFF3DA}} \color[HTML]{000000} 15 & {\cellcolor[HTML]{DBF1D5}} \color[HTML]{000000} 17 & {\cellcolor[HTML]{D8F0D2}} \color[HTML]{000000} 18 & {\cellcolor[HTML]{CEECC8}} \color[HTML]{000000} 22 & {\cellcolor[HTML]{CAEAC3}} \color[HTML]{000000} 24 & {\cellcolor[HTML]{C1E6BA}} \color[HTML]{000000} 27 & {\cellcolor[HTML]{B8E3B2}} \color[HTML]{000000} 30 & {\cellcolor[HTML]{ABDDA5}} \color[HTML]{000000} 34 & {\cellcolor[HTML]{B5E1AE}} \color[HTML]{000000} 31 & {\cellcolor[HTML]{ABDDA5}} \color[HTML]{000000} 34 & {\cellcolor[HTML]{A3DA9D}} \color[HTML]{000000} 37 & {\cellcolor[HTML]{95D391}} \color[HTML]{000000} 41 & {\cellcolor[HTML]{83CB82}} \color[HTML]{000000} 46 & {\cellcolor[HTML]{73C476}} \color[HTML]{000000} 50 & {\cellcolor[HTML]{63BC6E}} \color[HTML]{F1F1F1} 54 & {\cellcolor[HTML]{DDF2D8}} \color[HTML]{000000} 16 & {\cellcolor[HTML]{DBF1D5}} \color[HTML]{000000} 17 & {\cellcolor[HTML]{D8F0D2}} \color[HTML]{000000} 18 & {\cellcolor[HTML]{D3EECD}} \color[HTML]{000000} 20 & {\cellcolor[HTML]{CCEBC6}} \color[HTML]{000000} 23 & {\cellcolor[HTML]{C4E8BD}} \color[HTML]{000000} 26 & {\cellcolor[HTML]{B8E3B2}} \color[HTML]{000000} 30 & {\cellcolor[HTML]{ABDDA5}} \color[HTML]{000000} 34 & {\cellcolor[HTML]{A9DCA3}} \color[HTML]{000000} 35 & {\cellcolor[HTML]{A5DB9F}} \color[HTML]{000000} 36 & {\cellcolor[HTML]{9FD899}} \color[HTML]{000000} 38 & {\cellcolor[HTML]{95D391}} \color[HTML]{000000} 41 & {\cellcolor[HTML]{83CB82}} \color[HTML]{000000} 46 \\
BNCI2014001 & {\cellcolor[HTML]{95D391}} \color[HTML]{000000} 41 & {\cellcolor[HTML]{8DD08A}} \color[HTML]{000000} 43 & {\cellcolor[HTML]{86CC85}} \color[HTML]{000000} 45 & {\cellcolor[HTML]{7FC97F}} \color[HTML]{000000} 47 & {\cellcolor[HTML]{78C679}} \color[HTML]{000000} 49 & \bfseries {\cellcolor[HTML]{A5DB9F}} \color[HTML]{000000} 36 & \bfseries {\cellcolor[HTML]{95D391}} \color[HTML]{000000} 41 & \bfseries {\cellcolor[HTML]{7FC97F}} \color[HTML]{000000} 47 & \bfseries {\cellcolor[HTML]{6BC072}} \color[HTML]{000000} 52 & \bfseries {\cellcolor[HTML]{5BB86A}} \color[HTML]{F1F1F1} 56 & \bfseries {\cellcolor[HTML]{4EB264}} \color[HTML]{F1F1F1} 59 & \bfseries {\cellcolor[HTML]{D1EDCB}} \color[HTML]{000000} 21 & {\cellcolor[HTML]{D1EDCB}} \color[HTML]{000000} 21 & {\cellcolor[HTML]{CEECC8}} \color[HTML]{000000} 22 & \bfseries {\cellcolor[HTML]{CAEAC3}} \color[HTML]{000000} 24 & \bfseries {\cellcolor[HTML]{C7E9C0}} \color[HTML]{000000} 25 & \bfseries {\cellcolor[HTML]{C4E8BD}} \color[HTML]{000000} 26 & \bfseries {\cellcolor[HTML]{DFF3DA}} \color[HTML]{000000} 15 & {\cellcolor[HTML]{DFF3DA}} \color[HTML]{000000} 15 & {\cellcolor[HTML]{DDF2D8}} \color[HTML]{000000} 16 & \bfseries {\cellcolor[HTML]{DBF1D5}} \color[HTML]{000000} 17 & \bfseries {\cellcolor[HTML]{D8F0D2}} \color[HTML]{000000} 18 & \bfseries {\cellcolor[HTML]{D6EFD0}} \color[HTML]{000000} 19 & {\cellcolor[HTML]{CCEBC6}} \color[HTML]{000000} 23 & {\cellcolor[HTML]{C4E8BD}} \color[HTML]{000000} 26 & {\cellcolor[HTML]{B8E3B2}} \color[HTML]{000000} 30 & {\cellcolor[HTML]{ABDDA5}} \color[HTML]{000000} 34 & {\cellcolor[HTML]{9FD899}} \color[HTML]{000000} 38 & {\cellcolor[HTML]{9CD797}} \color[HTML]{000000} 39 & {\cellcolor[HTML]{8ACE88}} \color[HTML]{000000} 44 & {\cellcolor[HTML]{78C679}} \color[HTML]{000000} 49 & {\cellcolor[HTML]{63BC6E}} \color[HTML]{F1F1F1} 54 & {\cellcolor[HTML]{53B466}} \color[HTML]{F1F1F1} 58 & {\cellcolor[HTML]{43AC5E}} \color[HTML]{F1F1F1} 62 & {\cellcolor[HTML]{3BA458}} \color[HTML]{F1F1F1} 65 & {\cellcolor[HTML]{D8F0D2}} \color[HTML]{000000} 18 & {\cellcolor[HTML]{D3EECD}} \color[HTML]{000000} 20 & {\cellcolor[HTML]{CCEBC6}} \color[HTML]{000000} 23 & {\cellcolor[HTML]{BEE5B8}} \color[HTML]{000000} 28 & {\cellcolor[HTML]{B2E0AC}} \color[HTML]{000000} 32 & {\cellcolor[HTML]{9FD899}} \color[HTML]{000000} 38 & {\cellcolor[HTML]{8DD08A}} \color[HTML]{000000} 43 & {\cellcolor[HTML]{83CB82}} \color[HTML]{000000} 46 & {\cellcolor[HTML]{63BC6E}} \color[HTML]{F1F1F1} 54 & {\cellcolor[HTML]{4EB264}} \color[HTML]{F1F1F1} 59 & {\cellcolor[HTML]{3FA95C}} \color[HTML]{F1F1F1} 63 & {\cellcolor[HTML]{339C52}} \color[HTML]{F1F1F1} 68 & {\cellcolor[HTML]{2A924A}} \color[HTML]{F1F1F1} 72 \\
{\cellcolor[rgb]{.9,.9,.9}} BNCI2014004 & {\cellcolor[HTML]{9FD899}} \color[HTML]{000000} 38 & {\cellcolor[HTML]{95D391}} \color[HTML]{000000} 41 & {\cellcolor[HTML]{91D28E}} \color[HTML]{000000} 42 & {\cellcolor[HTML]{83CB82}} \color[HTML]{000000} 46 & {\cellcolor[HTML]{86CC85}} \color[HTML]{000000} 45 & {\cellcolor[HTML]{BBE4B4}} \color[HTML]{000000} 29 & {\cellcolor[HTML]{B2E0AC}} \color[HTML]{000000} 32 & {\cellcolor[HTML]{A9DCA3}} \color[HTML]{000000} 35 & {\cellcolor[HTML]{A3DA9D}} \color[HTML]{000000} 37 & {\cellcolor[HTML]{95D391}} \color[HTML]{000000} 41 & {\cellcolor[HTML]{8ACE88}} \color[HTML]{000000} 44 & {\cellcolor[HTML]{D3EECD}} \color[HTML]{000000} 20 & {\cellcolor[HTML]{D1EDCB}} \color[HTML]{000000} 21 & {\cellcolor[HTML]{D1EDCB}} \color[HTML]{000000} 21 & {\cellcolor[HTML]{CCEBC6}} \color[HTML]{000000} 23 & {\cellcolor[HTML]{CCEBC6}} \color[HTML]{000000} 23 & {\cellcolor[HTML]{CAEAC3}} \color[HTML]{000000} 24 & {\cellcolor[HTML]{E2F4DD}} \color[HTML]{000000} 14 & {\cellcolor[HTML]{E2F4DD}} \color[HTML]{000000} 14 & {\cellcolor[HTML]{DFF3DA}} \color[HTML]{000000} 15 & {\cellcolor[HTML]{DFF3DA}} \color[HTML]{000000} 15 & {\cellcolor[HTML]{DFF3DA}} \color[HTML]{000000} 15 & {\cellcolor[HTML]{DDF2D8}} \color[HTML]{000000} 16 & {\cellcolor[HTML]{D1EDCB}} \color[HTML]{000000} 21 & {\cellcolor[HTML]{CCEBC6}} \color[HTML]{000000} 23 & {\cellcolor[HTML]{C7E9C0}} \color[HTML]{000000} 25 & {\cellcolor[HTML]{BEE5B8}} \color[HTML]{000000} 28 & {\cellcolor[HTML]{B5E1AE}} \color[HTML]{000000} 31 & {\cellcolor[HTML]{A5DB9F}} \color[HTML]{000000} 36 & {\cellcolor[HTML]{95D391}} \color[HTML]{000000} 41 & {\cellcolor[HTML]{86CC85}} \color[HTML]{000000} 45 & {\cellcolor[HTML]{78C679}} \color[HTML]{000000} 49 & {\cellcolor[HTML]{68BE70}} \color[HTML]{000000} 53 & {\cellcolor[HTML]{5BB86A}} \color[HTML]{F1F1F1} 56 & {\cellcolor[HTML]{4BB062}} \color[HTML]{F1F1F1} 60 & {\cellcolor[HTML]{D8F0D2}} \color[HTML]{000000} 18 & {\cellcolor[HTML]{D3EECD}} \color[HTML]{000000} 20 & {\cellcolor[HTML]{CEECC8}} \color[HTML]{000000} 22 & {\cellcolor[HTML]{C4E8BD}} \color[HTML]{000000} 26 & {\cellcolor[HTML]{BBE4B4}} \color[HTML]{000000} 29 & {\cellcolor[HTML]{AFDFA8}} \color[HTML]{000000} 33 & {\cellcolor[HTML]{A5DB9F}} \color[HTML]{000000} 36 & {\cellcolor[HTML]{7CC87C}} \color[HTML]{000000} 48 & {\cellcolor[HTML]{63BC6E}} \color[HTML]{F1F1F1} 54 & {\cellcolor[HTML]{46AE60}} \color[HTML]{F1F1F1} 61 & {\cellcolor[HTML]{3EA75A}} \color[HTML]{F1F1F1} 64 & {\cellcolor[HTML]{339C52}} \color[HTML]{F1F1F1} 68 & {\cellcolor[HTML]{2A924A}} \color[HTML]{F1F1F1} 72 \\
BNCI2015001 & {\cellcolor[HTML]{98D594}} \color[HTML]{000000} 40 & {\cellcolor[HTML]{8DD08A}} \color[HTML]{000000} 43 & {\cellcolor[HTML]{83CB82}} \color[HTML]{000000} 46 & {\cellcolor[HTML]{7CC87C}} \color[HTML]{000000} 48 & {\cellcolor[HTML]{7CC87C}} \color[HTML]{000000} 48 & {\cellcolor[HTML]{ABDDA5}} \color[HTML]{000000} 34 & {\cellcolor[HTML]{A3DA9D}} \color[HTML]{000000} 37 & {\cellcolor[HTML]{98D594}} \color[HTML]{000000} 40 & {\cellcolor[HTML]{8DD08A}} \color[HTML]{000000} 43 & {\cellcolor[HTML]{7FC97F}} \color[HTML]{000000} 47 & {\cellcolor[HTML]{73C476}} \color[HTML]{000000} 50 & {\cellcolor[HTML]{D3EECD}} \color[HTML]{000000} 20 & {\cellcolor[HTML]{D3EECD}} \color[HTML]{000000} 20 & {\cellcolor[HTML]{D1EDCB}} \color[HTML]{000000} 21 & {\cellcolor[HTML]{CCEBC6}} \color[HTML]{000000} 23 & {\cellcolor[HTML]{CCEBC6}} \color[HTML]{000000} 23 & {\cellcolor[HTML]{C7E9C0}} \color[HTML]{000000} 25 & \bfseries {\cellcolor[HTML]{DFF3DA}} \color[HTML]{000000} 15 & \bfseries {\cellcolor[HTML]{DDF2D8}} \color[HTML]{000000} 16 & \bfseries {\cellcolor[HTML]{DBF1D5}} \color[HTML]{000000} 17 & \bfseries {\cellcolor[HTML]{DBF1D5}} \color[HTML]{000000} 17 & \bfseries {\cellcolor[HTML]{D8F0D2}} \color[HTML]{000000} 18 & {\cellcolor[HTML]{D8F0D2}} \color[HTML]{000000} 18 & {\cellcolor[HTML]{CEECC8}} \color[HTML]{000000} 22 & {\cellcolor[HTML]{C7E9C0}} \color[HTML]{000000} 25 & {\cellcolor[HTML]{BEE5B8}} \color[HTML]{000000} 28 & {\cellcolor[HTML]{B5E1AE}} \color[HTML]{000000} 31 & {\cellcolor[HTML]{ABDDA5}} \color[HTML]{000000} 34 & {\cellcolor[HTML]{A5DB9F}} \color[HTML]{000000} 36 & {\cellcolor[HTML]{95D391}} \color[HTML]{000000} 41 & {\cellcolor[HTML]{86CC85}} \color[HTML]{000000} 45 & {\cellcolor[HTML]{78C679}} \color[HTML]{000000} 49 & {\cellcolor[HTML]{68BE70}} \color[HTML]{000000} 53 & {\cellcolor[HTML]{58B668}} \color[HTML]{F1F1F1} 57 & {\cellcolor[HTML]{46AE60}} \color[HTML]{F1F1F1} 61 & {\cellcolor[HTML]{D6EFD0}} \color[HTML]{000000} 19 & {\cellcolor[HTML]{D1EDCB}} \color[HTML]{000000} 21 & {\cellcolor[HTML]{CAEAC3}} \color[HTML]{000000} 24 & {\cellcolor[HTML]{C1E6BA}} \color[HTML]{000000} 27 & {\cellcolor[HTML]{B8E3B2}} \color[HTML]{000000} 30 & {\cellcolor[HTML]{A9DCA3}} \color[HTML]{000000} 35 & {\cellcolor[HTML]{9CD797}} \color[HTML]{000000} 39 & {\cellcolor[HTML]{86CC85}} \color[HTML]{000000} 45 & {\cellcolor[HTML]{73C476}} \color[HTML]{000000} 50 & {\cellcolor[HTML]{60BA6C}} \color[HTML]{F1F1F1} 55 & {\cellcolor[HTML]{4EB264}} \color[HTML]{F1F1F1} 59 & {\cellcolor[HTML]{3FA95C}} \color[HTML]{F1F1F1} 63 & {\cellcolor[HTML]{39A257}} \color[HTML]{F1F1F1} 66 \\
{\cellcolor[rgb]{.9,.9,.9}} BNCI2015004 & {\cellcolor[HTML]{ABDDA5}} \color[HTML]{000000} 34 & {\cellcolor[HTML]{B2E0AC}} \color[HTML]{000000} 32 & {\cellcolor[HTML]{B2E0AC}} \color[HTML]{000000} 32 & {\cellcolor[HTML]{AFDFA8}} \color[HTML]{000000} 33 & {\cellcolor[HTML]{ABDDA5}} \color[HTML]{000000} 34 & {\cellcolor[HTML]{C1E6BA}} \color[HTML]{000000} 27 & {\cellcolor[HTML]{BEE5B8}} \color[HTML]{000000} 28 & {\cellcolor[HTML]{BBE4B4}} \color[HTML]{000000} 29 & {\cellcolor[HTML]{B5E1AE}} \color[HTML]{000000} 31 & {\cellcolor[HTML]{ABDDA5}} \color[HTML]{000000} 34 & {\cellcolor[HTML]{9FD899}} \color[HTML]{000000} 38 & {\cellcolor[HTML]{D3EECD}} \color[HTML]{000000} 20 & {\cellcolor[HTML]{D3EECD}} \color[HTML]{000000} 20 & {\cellcolor[HTML]{D1EDCB}} \color[HTML]{000000} 21 & {\cellcolor[HTML]{CEECC8}} \color[HTML]{000000} 22 & {\cellcolor[HTML]{CCEBC6}} \color[HTML]{000000} 23 & {\cellcolor[HTML]{CCEBC6}} \color[HTML]{000000} 23 & {\cellcolor[HTML]{E2F4DD}} \color[HTML]{000000} 14 & {\cellcolor[HTML]{E2F4DD}} \color[HTML]{000000} 14 & {\cellcolor[HTML]{DFF3DA}} \color[HTML]{000000} 15 & {\cellcolor[HTML]{DFF3DA}} \color[HTML]{000000} 15 & {\cellcolor[HTML]{DDF2D8}} \color[HTML]{000000} 16 & {\cellcolor[HTML]{DBF1D5}} \color[HTML]{000000} 17 & {\cellcolor[HTML]{CEECC8}} \color[HTML]{000000} 22 & {\cellcolor[HTML]{CAEAC3}} \color[HTML]{000000} 24 & {\cellcolor[HTML]{C4E8BD}} \color[HTML]{000000} 26 & {\cellcolor[HTML]{BBE4B4}} \color[HTML]{000000} 29 & {\cellcolor[HTML]{B2E0AC}} \color[HTML]{000000} 32 & {\cellcolor[HTML]{B8E3B2}} \color[HTML]{000000} 30 & {\cellcolor[HTML]{B5E1AE}} \color[HTML]{000000} 31 & {\cellcolor[HTML]{ABDDA5}} \color[HTML]{000000} 34 & {\cellcolor[HTML]{9FD899}} \color[HTML]{000000} 38 & {\cellcolor[HTML]{8DD08A}} \color[HTML]{000000} 43 & {\cellcolor[HTML]{7FC97F}} \color[HTML]{000000} 47 & {\cellcolor[HTML]{70C274}} \color[HTML]{000000} 51 & {\cellcolor[HTML]{DDF2D8}} \color[HTML]{000000} 16 & {\cellcolor[HTML]{DDF2D8}} \color[HTML]{000000} 16 & {\cellcolor[HTML]{D8F0D2}} \color[HTML]{000000} 18 & {\cellcolor[HTML]{D6EFD0}} \color[HTML]{000000} 19 & {\cellcolor[HTML]{CEECC8}} \color[HTML]{000000} 22 & {\cellcolor[HTML]{C7E9C0}} \color[HTML]{000000} 25 & {\cellcolor[HTML]{BBE4B4}} \color[HTML]{000000} 29 & {\cellcolor[HTML]{ABDDA5}} \color[HTML]{000000} 34 & {\cellcolor[HTML]{A9DCA3}} \color[HTML]{000000} 35 & {\cellcolor[HTML]{A5DB9F}} \color[HTML]{000000} 36 & {\cellcolor[HTML]{9FD899}} \color[HTML]{000000} 38 & {\cellcolor[HTML]{95D391}} \color[HTML]{000000} 41 & {\cellcolor[HTML]{86CC85}} \color[HTML]{000000} 45 \\
Cho2017 & {\cellcolor[HTML]{A9DCA3}} \color[HTML]{000000} 35 & {\cellcolor[HTML]{AFDFA8}} \color[HTML]{000000} 33 & {\cellcolor[HTML]{AFDFA8}} \color[HTML]{000000} 33 & {\cellcolor[HTML]{A9DCA3}} \color[HTML]{000000} 35 & {\cellcolor[HTML]{A5DB9F}} \color[HTML]{000000} 36 & {\cellcolor[HTML]{C1E6BA}} \color[HTML]{000000} 27 & {\cellcolor[HTML]{BEE5B8}} \color[HTML]{000000} 28 & {\cellcolor[HTML]{B8E3B2}} \color[HTML]{000000} 30 & {\cellcolor[HTML]{B2E0AC}} \color[HTML]{000000} 32 & {\cellcolor[HTML]{ABDDA5}} \color[HTML]{000000} 34 & {\cellcolor[HTML]{A3DA9D}} \color[HTML]{000000} 37 & {\cellcolor[HTML]{D3EECD}} \color[HTML]{000000} 20 & {\cellcolor[HTML]{D3EECD}} \color[HTML]{000000} 20 & {\cellcolor[HTML]{D3EECD}} \color[HTML]{000000} 20 & {\cellcolor[HTML]{D3EECD}} \color[HTML]{000000} 20 & {\cellcolor[HTML]{D1EDCB}} \color[HTML]{000000} 21 & {\cellcolor[HTML]{CEECC8}} \color[HTML]{000000} 22 & {\cellcolor[HTML]{E2F4DD}} \color[HTML]{000000} 14 & {\cellcolor[HTML]{E2F4DD}} \color[HTML]{000000} 14 & {\cellcolor[HTML]{DFF3DA}} \color[HTML]{000000} 15 & {\cellcolor[HTML]{DFF3DA}} \color[HTML]{000000} 15 & {\cellcolor[HTML]{DDF2D8}} \color[HTML]{000000} 16 & {\cellcolor[HTML]{DBF1D5}} \color[HTML]{000000} 17 & {\cellcolor[HTML]{CEECC8}} \color[HTML]{000000} 22 & {\cellcolor[HTML]{CCEBC6}} \color[HTML]{000000} 23 & {\cellcolor[HTML]{C7E9C0}} \color[HTML]{000000} 25 & {\cellcolor[HTML]{BEE5B8}} \color[HTML]{000000} 28 & {\cellcolor[HTML]{B5E1AE}} \color[HTML]{000000} 31 & {\cellcolor[HTML]{BEE5B8}} \color[HTML]{000000} 28 & {\cellcolor[HTML]{B8E3B2}} \color[HTML]{000000} 30 & {\cellcolor[HTML]{B2E0AC}} \color[HTML]{000000} 32 & {\cellcolor[HTML]{ABDDA5}} \color[HTML]{000000} 34 & {\cellcolor[HTML]{A3DA9D}} \color[HTML]{000000} 37 & {\cellcolor[HTML]{95D391}} \color[HTML]{000000} 41 & {\cellcolor[HTML]{8ACE88}} \color[HTML]{000000} 44 & {\cellcolor[HTML]{DDF2D8}} \color[HTML]{000000} 16 & {\cellcolor[HTML]{DDF2D8}} \color[HTML]{000000} 16 & {\cellcolor[HTML]{DBF1D5}} \color[HTML]{000000} 17 & {\cellcolor[HTML]{D8F0D2}} \color[HTML]{000000} 18 & {\cellcolor[HTML]{D3EECD}} \color[HTML]{000000} 20 & {\cellcolor[HTML]{D1EDCB}} \color[HTML]{000000} 21 & {\cellcolor[HTML]{CCEBC6}} \color[HTML]{000000} 23 & {\cellcolor[HTML]{A5DB9F}} \color[HTML]{000000} 36 & {\cellcolor[HTML]{9FD899}} \color[HTML]{000000} 38 & {\cellcolor[HTML]{98D594}} \color[HTML]{000000} 40 & {\cellcolor[HTML]{8DD08A}} \color[HTML]{000000} 43 & {\cellcolor[HTML]{83CB82}} \color[HTML]{000000} 46 & {\cellcolor[HTML]{78C679}} \color[HTML]{000000} 49 \\
{\cellcolor[rgb]{.9,.9,.9}} Lee2019\_MI & {\cellcolor[HTML]{A3DA9D}} \color[HTML]{000000} 37 & {\cellcolor[HTML]{9CD797}} \color[HTML]{000000} 39 & {\cellcolor[HTML]{8ACE88}} \color[HTML]{000000} 44 & {\cellcolor[HTML]{7FC97F}} \color[HTML]{000000} 47 & {\cellcolor[HTML]{7CC87C}} \color[HTML]{000000} 48 & {\cellcolor[HTML]{AFDFA8}} \color[HTML]{000000} 33 & {\cellcolor[HTML]{A3DA9D}} \color[HTML]{000000} 37 & {\cellcolor[HTML]{95D391}} \color[HTML]{000000} 41 & {\cellcolor[HTML]{8DD08A}} \color[HTML]{000000} 43 & {\cellcolor[HTML]{7FC97F}} \color[HTML]{000000} 47 & {\cellcolor[HTML]{70C274}} \color[HTML]{000000} 51 & {\cellcolor[HTML]{D3EECD}} \color[HTML]{000000} 20 & {\cellcolor[HTML]{D1EDCB}} \color[HTML]{000000} 21 & {\cellcolor[HTML]{D1EDCB}} \color[HTML]{000000} 21 & {\cellcolor[HTML]{D1EDCB}} \color[HTML]{000000} 21 & {\cellcolor[HTML]{CCEBC6}} \color[HTML]{000000} 23 & {\cellcolor[HTML]{CCEBC6}} \color[HTML]{000000} 23 & {\cellcolor[HTML]{E2F4DD}} \color[HTML]{000000} 14 & {\cellcolor[HTML]{DFF3DA}} \color[HTML]{000000} 15 & {\cellcolor[HTML]{DDF2D8}} \color[HTML]{000000} 16 & \bfseries {\cellcolor[HTML]{DBF1D5}} \color[HTML]{000000} 17 & {\cellcolor[HTML]{DBF1D5}} \color[HTML]{000000} 17 & {\cellcolor[HTML]{DBF1D5}} \color[HTML]{000000} 17 & {\cellcolor[HTML]{CEECC8}} \color[HTML]{000000} 22 & {\cellcolor[HTML]{CAEAC3}} \color[HTML]{000000} 24 & {\cellcolor[HTML]{C1E6BA}} \color[HTML]{000000} 27 & {\cellcolor[HTML]{B8E3B2}} \color[HTML]{000000} 30 & {\cellcolor[HTML]{AFDFA8}} \color[HTML]{000000} 33 & {\cellcolor[HTML]{ABDDA5}} \color[HTML]{000000} 34 & {\cellcolor[HTML]{9FD899}} \color[HTML]{000000} 38 & {\cellcolor[HTML]{8ACE88}} \color[HTML]{000000} 44 & {\cellcolor[HTML]{78C679}} \color[HTML]{000000} 49 & {\cellcolor[HTML]{68BE70}} \color[HTML]{000000} 53 & {\cellcolor[HTML]{53B466}} \color[HTML]{F1F1F1} 58 & {\cellcolor[HTML]{43AC5E}} \color[HTML]{F1F1F1} 62 & {\cellcolor[HTML]{D6EFD0}} \color[HTML]{000000} 19 & {\cellcolor[HTML]{CEECC8}} \color[HTML]{000000} 22 & {\cellcolor[HTML]{C7E9C0}} \color[HTML]{000000} 25 & {\cellcolor[HTML]{BEE5B8}} \color[HTML]{000000} 28 & {\cellcolor[HTML]{B2E0AC}} \color[HTML]{000000} 32 & {\cellcolor[HTML]{A3DA9D}} \color[HTML]{000000} 37 & {\cellcolor[HTML]{95D391}} \color[HTML]{000000} 41 & {\cellcolor[HTML]{6BC072}} \color[HTML]{000000} 52 & {\cellcolor[HTML]{4BB062}} \color[HTML]{F1F1F1} 60 & {\cellcolor[HTML]{39A257}} \color[HTML]{F1F1F1} 66 & {\cellcolor[HTML]{2F974E}} \color[HTML]{F1F1F1} 70 & {\cellcolor[HTML]{258D47}} \color[HTML]{F1F1F1} 74 & {\cellcolor[HTML]{1D8640}} \color[HTML]{F1F1F1} 77 \\
Ofner2017(I) & {\cellcolor[HTML]{AFDFA8}} \color[HTML]{000000} 33 & {\cellcolor[HTML]{AFDFA8}} \color[HTML]{000000} 33 & {\cellcolor[HTML]{AFDFA8}} \color[HTML]{000000} 33 & {\cellcolor[HTML]{AFDFA8}} \color[HTML]{000000} 33 & {\cellcolor[HTML]{AFDFA8}} \color[HTML]{000000} 33 & {\cellcolor[HTML]{CAEAC3}} \color[HTML]{000000} 24 & {\cellcolor[HTML]{CAEAC3}} \color[HTML]{000000} 24 & {\cellcolor[HTML]{CAEAC3}} \color[HTML]{000000} 24 & {\cellcolor[HTML]{CAEAC3}} \color[HTML]{000000} 24 & {\cellcolor[HTML]{CAEAC3}} \color[HTML]{000000} 24 & {\cellcolor[HTML]{CAEAC3}} \color[HTML]{000000} 24 & {\cellcolor[HTML]{D3EECD}} \color[HTML]{000000} 20 & {\cellcolor[HTML]{D3EECD}} \color[HTML]{000000} 20 & {\cellcolor[HTML]{D3EECD}} \color[HTML]{000000} 20 & {\cellcolor[HTML]{D3EECD}} \color[HTML]{000000} 20 & {\cellcolor[HTML]{D3EECD}} \color[HTML]{000000} 20 & {\cellcolor[HTML]{D3EECD}} \color[HTML]{000000} 20 & {\cellcolor[HTML]{E2F4DD}} \color[HTML]{000000} 14 & {\cellcolor[HTML]{DFF3DA}} \color[HTML]{000000} 15 & {\cellcolor[HTML]{DFF3DA}} \color[HTML]{000000} 15 & {\cellcolor[HTML]{DDF2D8}} \color[HTML]{000000} 16 & {\cellcolor[HTML]{DBF1D5}} \color[HTML]{000000} 17 & {\cellcolor[HTML]{D8F0D2}} \color[HTML]{000000} 18 & {\cellcolor[HTML]{E6F5E1}} \color[HTML]{000000} 12 & {\cellcolor[HTML]{E6F5E1}} \color[HTML]{000000} 12 & {\cellcolor[HTML]{E6F5E1}} \color[HTML]{000000} 12 & {\cellcolor[HTML]{E6F5E1}} \color[HTML]{000000} 12 & {\cellcolor[HTML]{E6F5E1}} \color[HTML]{000000} 12 & {\cellcolor[HTML]{C7E9C0}} \color[HTML]{000000} 25 & {\cellcolor[HTML]{C7E9C0}} \color[HTML]{000000} 25 & {\cellcolor[HTML]{C7E9C0}} \color[HTML]{000000} 25 & {\cellcolor[HTML]{C7E9C0}} \color[HTML]{000000} 25 & {\cellcolor[HTML]{C7E9C0}} \color[HTML]{000000} 25 & {\cellcolor[HTML]{C7E9C0}} \color[HTML]{000000} 25 & {\cellcolor[HTML]{C7E9C0}} \color[HTML]{000000} 25 & {\cellcolor[HTML]{E2F4DD}} \color[HTML]{000000} 14 & {\cellcolor[HTML]{E2F4DD}} \color[HTML]{000000} 14 & {\cellcolor[HTML]{E2F4DD}} \color[HTML]{000000} 14 & {\cellcolor[HTML]{E2F4DD}} \color[HTML]{000000} 14 & {\cellcolor[HTML]{E2F4DD}} \color[HTML]{000000} 14 & {\cellcolor[HTML]{E2F4DD}} \color[HTML]{000000} 14 & {\cellcolor[HTML]{E2F4DD}} \color[HTML]{000000} 14 & {\cellcolor[HTML]{AFDFA8}} \color[HTML]{000000} 33 & {\cellcolor[HTML]{AFDFA8}} \color[HTML]{000000} 33 & {\cellcolor[HTML]{AFDFA8}} \color[HTML]{000000} 33 & {\cellcolor[HTML]{AFDFA8}} \color[HTML]{000000} 33 & {\cellcolor[HTML]{AFDFA8}} \color[HTML]{000000} 33 & {\cellcolor[HTML]{AFDFA8}} \color[HTML]{000000} 33 \\
{\cellcolor[rgb]{.9,.9,.9}} PhysionetMI(I,E) & \bfseries {\cellcolor[HTML]{8ACE88}} \color[HTML]{000000} 44 & \bfseries {\cellcolor[HTML]{78C679}} \color[HTML]{000000} 49 & \bfseries {\cellcolor[HTML]{78C679}} \color[HTML]{000000} 49 & \bfseries {\cellcolor[HTML]{70C274}} \color[HTML]{000000} 51 & \bfseries {\cellcolor[HTML]{5BB86A}} \color[HTML]{F1F1F1} 56 & {\cellcolor[HTML]{A9DCA3}} \color[HTML]{000000} 35 & {\cellcolor[HTML]{9CD797}} \color[HTML]{000000} 39 & {\cellcolor[HTML]{8DD08A}} \color[HTML]{000000} 43 & {\cellcolor[HTML]{7FC97F}} \color[HTML]{000000} 47 & {\cellcolor[HTML]{70C274}} \color[HTML]{000000} 51 & {\cellcolor[HTML]{5BB86A}} \color[HTML]{F1F1F1} 56 & \bfseries {\cellcolor[HTML]{D1EDCB}} \color[HTML]{000000} 21 & \bfseries {\cellcolor[HTML]{CEECC8}} \color[HTML]{000000} 22 & \bfseries {\cellcolor[HTML]{CCEBC6}} \color[HTML]{000000} 23 & \bfseries {\cellcolor[HTML]{CAEAC3}} \color[HTML]{000000} 24 & \bfseries {\cellcolor[HTML]{C7E9C0}} \color[HTML]{000000} 25 & \bfseries {\cellcolor[HTML]{C4E8BD}} \color[HTML]{000000} 26 & \bfseries {\cellcolor[HTML]{DFF3DA}} \color[HTML]{000000} 15 & {\cellcolor[HTML]{DFF3DA}} \color[HTML]{000000} 15 & {\cellcolor[HTML]{DDF2D8}} \color[HTML]{000000} 16 & {\cellcolor[HTML]{DDF2D8}} \color[HTML]{000000} 16 & {\cellcolor[HTML]{DBF1D5}} \color[HTML]{000000} 17 & {\cellcolor[HTML]{DBF1D5}} \color[HTML]{000000} 17 & \bfseries {\cellcolor[HTML]{C7E9C0}} \color[HTML]{000000} 25 & \bfseries {\cellcolor[HTML]{BBE4B4}} \color[HTML]{000000} 29 & \bfseries {\cellcolor[HTML]{ABDDA5}} \color[HTML]{000000} 34 & \bfseries {\cellcolor[HTML]{9FD899}} \color[HTML]{000000} 38 & \bfseries {\cellcolor[HTML]{8DD08A}} \color[HTML]{000000} 43 & {\cellcolor[HTML]{95D391}} \color[HTML]{000000} 41 & {\cellcolor[HTML]{83CB82}} \color[HTML]{000000} 46 & {\cellcolor[HTML]{70C274}} \color[HTML]{000000} 51 & {\cellcolor[HTML]{5BB86A}} \color[HTML]{F1F1F1} 56 & {\cellcolor[HTML]{4BB062}} \color[HTML]{F1F1F1} 60 & {\cellcolor[HTML]{3EA75A}} \color[HTML]{F1F1F1} 64 & {\cellcolor[HTML]{319A50}} \color[HTML]{F1F1F1} 69 & \bfseries {\cellcolor[HTML]{D3EECD}} \color[HTML]{000000} 20 & \bfseries {\cellcolor[HTML]{CCEBC6}} \color[HTML]{000000} 23 & \bfseries {\cellcolor[HTML]{C4E8BD}} \color[HTML]{000000} 26 & \bfseries {\cellcolor[HTML]{B8E3B2}} \color[HTML]{000000} 30 & \bfseries {\cellcolor[HTML]{A5DB9F}} \color[HTML]{000000} 36 & \bfseries {\cellcolor[HTML]{95D391}} \color[HTML]{000000} 41 & \bfseries {\cellcolor[HTML]{83CB82}} \color[HTML]{000000} 46 & {\cellcolor[HTML]{83CB82}} \color[HTML]{000000} 46 & {\cellcolor[HTML]{6BC072}} \color[HTML]{000000} 52 & {\cellcolor[HTML]{53B466}} \color[HTML]{F1F1F1} 58 & {\cellcolor[HTML]{43AC5E}} \color[HTML]{F1F1F1} 62 & {\cellcolor[HTML]{369F54}} \color[HTML]{F1F1F1} 67 & {\cellcolor[HTML]{2A924A}} \color[HTML]{F1F1F1} 72 \\
Schirrmeister2017 & {\cellcolor[HTML]{95D391}} \color[HTML]{000000} 41 & {\cellcolor[HTML]{8ACE88}} \color[HTML]{000000} 44 & {\cellcolor[HTML]{7CC87C}} \color[HTML]{000000} 48 & {\cellcolor[HTML]{73C476}} \color[HTML]{000000} 50 & {\cellcolor[HTML]{63BC6E}} \color[HTML]{F1F1F1} 54 & {\cellcolor[HTML]{ABDDA5}} \color[HTML]{000000} 34 & {\cellcolor[HTML]{9FD899}} \color[HTML]{000000} 38 & {\cellcolor[HTML]{91D28E}} \color[HTML]{000000} 42 & {\cellcolor[HTML]{83CB82}} \color[HTML]{000000} 46 & {\cellcolor[HTML]{73C476}} \color[HTML]{000000} 50 & {\cellcolor[HTML]{63BC6E}} \color[HTML]{F1F1F1} 54 & \bfseries {\cellcolor[HTML]{D1EDCB}} \color[HTML]{000000} 21 & {\cellcolor[HTML]{D1EDCB}} \color[HTML]{000000} 21 & {\cellcolor[HTML]{CEECC8}} \color[HTML]{000000} 22 & {\cellcolor[HTML]{CEECC8}} \color[HTML]{000000} 22 & {\cellcolor[HTML]{CCEBC6}} \color[HTML]{000000} 23 & {\cellcolor[HTML]{CAEAC3}} \color[HTML]{000000} 24 & \bfseries {\cellcolor[HTML]{DFF3DA}} \color[HTML]{000000} 15 & {\cellcolor[HTML]{DFF3DA}} \color[HTML]{000000} 15 & {\cellcolor[HTML]{DDF2D8}} \color[HTML]{000000} 16 & {\cellcolor[HTML]{DDF2D8}} \color[HTML]{000000} 16 & {\cellcolor[HTML]{DBF1D5}} \color[HTML]{000000} 17 & {\cellcolor[HTML]{DBF1D5}} \color[HTML]{000000} 17 & {\cellcolor[HTML]{CCEBC6}} \color[HTML]{000000} 23 & {\cellcolor[HTML]{C4E8BD}} \color[HTML]{000000} 26 & {\cellcolor[HTML]{BEE5B8}} \color[HTML]{000000} 28 & {\cellcolor[HTML]{B5E1AE}} \color[HTML]{000000} 31 & {\cellcolor[HTML]{A9DCA3}} \color[HTML]{000000} 35 & \bfseries {\cellcolor[HTML]{86CC85}} \color[HTML]{000000} 45 & \bfseries {\cellcolor[HTML]{6BC072}} \color[HTML]{000000} 52 & \bfseries {\cellcolor[HTML]{58B668}} \color[HTML]{F1F1F1} 57 & \bfseries {\cellcolor[HTML]{43AC5E}} \color[HTML]{F1F1F1} 62 & \bfseries {\cellcolor[HTML]{39A257}} \color[HTML]{F1F1F1} 66 & \bfseries {\cellcolor[HTML]{2F974E}} \color[HTML]{F1F1F1} 70 & \bfseries {\cellcolor[HTML]{289049}} \color[HTML]{F1F1F1} 73 & {\cellcolor[HTML]{D8F0D2}} \color[HTML]{000000} 18 & {\cellcolor[HTML]{D1EDCB}} \color[HTML]{000000} 21 & {\cellcolor[HTML]{C7E9C0}} \color[HTML]{000000} 25 & {\cellcolor[HTML]{BEE5B8}} \color[HTML]{000000} 28 & {\cellcolor[HTML]{AFDFA8}} \color[HTML]{000000} 33 & {\cellcolor[HTML]{9FD899}} \color[HTML]{000000} 38 & {\cellcolor[HTML]{91D28E}} \color[HTML]{000000} 42 & {\cellcolor[HTML]{78C679}} \color[HTML]{000000} 49 & {\cellcolor[HTML]{60BA6C}} \color[HTML]{F1F1F1} 55 & {\cellcolor[HTML]{4BB062}} \color[HTML]{F1F1F1} 60 & {\cellcolor[HTML]{39A257}} \color[HTML]{F1F1F1} 66 & {\cellcolor[HTML]{319A50}} \color[HTML]{F1F1F1} 69 & {\cellcolor[HTML]{289049}} \color[HTML]{F1F1F1} 73 \\
{\cellcolor[rgb]{.9,.9,.9}} Weibo2014 & {\cellcolor[HTML]{91D28E}} \color[HTML]{000000} 42 & {\cellcolor[HTML]{8DD08A}} \color[HTML]{000000} 43 & {\cellcolor[HTML]{86CC85}} \color[HTML]{000000} 45 & {\cellcolor[HTML]{86CC85}} \color[HTML]{000000} 45 & {\cellcolor[HTML]{83CB82}} \color[HTML]{000000} 46 & {\cellcolor[HTML]{AFDFA8}} \color[HTML]{000000} 33 & {\cellcolor[HTML]{A9DCA3}} \color[HTML]{000000} 35 & {\cellcolor[HTML]{9FD899}} \color[HTML]{000000} 38 & {\cellcolor[HTML]{95D391}} \color[HTML]{000000} 41 & {\cellcolor[HTML]{83CB82}} \color[HTML]{000000} 46 & {\cellcolor[HTML]{73C476}} \color[HTML]{000000} 50 & \bfseries {\cellcolor[HTML]{D1EDCB}} \color[HTML]{000000} 21 & {\cellcolor[HTML]{D1EDCB}} \color[HTML]{000000} 21 & {\cellcolor[HTML]{CEECC8}} \color[HTML]{000000} 22 & {\cellcolor[HTML]{CEECC8}} \color[HTML]{000000} 22 & {\cellcolor[HTML]{CCEBC6}} \color[HTML]{000000} 23 & {\cellcolor[HTML]{CAEAC3}} \color[HTML]{000000} 24 & \bfseries {\cellcolor[HTML]{DFF3DA}} \color[HTML]{000000} 15 & {\cellcolor[HTML]{DFF3DA}} \color[HTML]{000000} 15 & {\cellcolor[HTML]{DDF2D8}} \color[HTML]{000000} 16 & \bfseries {\cellcolor[HTML]{DBF1D5}} \color[HTML]{000000} 17 & \bfseries {\cellcolor[HTML]{D8F0D2}} \color[HTML]{000000} 18 & \bfseries {\cellcolor[HTML]{D6EFD0}} \color[HTML]{000000} 19 & {\cellcolor[HTML]{CCEBC6}} \color[HTML]{000000} 23 & {\cellcolor[HTML]{C4E8BD}} \color[HTML]{000000} 26 & {\cellcolor[HTML]{BBE4B4}} \color[HTML]{000000} 29 & {\cellcolor[HTML]{AFDFA8}} \color[HTML]{000000} 33 & {\cellcolor[HTML]{9FD899}} \color[HTML]{000000} 38 & {\cellcolor[HTML]{A9DCA3}} \color[HTML]{000000} 35 & {\cellcolor[HTML]{98D594}} \color[HTML]{000000} 40 & {\cellcolor[HTML]{86CC85}} \color[HTML]{000000} 45 & {\cellcolor[HTML]{78C679}} \color[HTML]{000000} 49 & {\cellcolor[HTML]{63BC6E}} \color[HTML]{F1F1F1} 54 & {\cellcolor[HTML]{53B466}} \color[HTML]{F1F1F1} 58 & {\cellcolor[HTML]{43AC5E}} \color[HTML]{F1F1F1} 62 & {\cellcolor[HTML]{DBF1D5}} \color[HTML]{000000} 17 & {\cellcolor[HTML]{D6EFD0}} \color[HTML]{000000} 19 & {\cellcolor[HTML]{CCEBC6}} \color[HTML]{000000} 23 & {\cellcolor[HTML]{C4E8BD}} \color[HTML]{000000} 26 & {\cellcolor[HTML]{B5E1AE}} \color[HTML]{000000} 31 & {\cellcolor[HTML]{ABDDA5}} \color[HTML]{000000} 34 & {\cellcolor[HTML]{9CD797}} \color[HTML]{000000} 39 & {\cellcolor[HTML]{8DD08A}} \color[HTML]{000000} 43 & {\cellcolor[HTML]{83CB82}} \color[HTML]{000000} 46 & {\cellcolor[HTML]{73C476}} \color[HTML]{000000} 50 & {\cellcolor[HTML]{68BE70}} \color[HTML]{000000} 53 & {\cellcolor[HTML]{60BA6C}} \color[HTML]{F1F1F1} 55 & {\cellcolor[HTML]{4EB264}} \color[HTML]{F1F1F1} 59 \\
Zhou2016 & {\cellcolor[HTML]{98D594}} \color[HTML]{000000} 40 & {\cellcolor[HTML]{91D28E}} \color[HTML]{000000} 42 & {\cellcolor[HTML]{86CC85}} \color[HTML]{000000} 45 & {\cellcolor[HTML]{7FC97F}} \color[HTML]{000000} 47 & {\cellcolor[HTML]{78C679}} \color[HTML]{000000} 49 & {\cellcolor[HTML]{AFDFA8}} \color[HTML]{000000} 33 & {\cellcolor[HTML]{A5DB9F}} \color[HTML]{000000} 36 & {\cellcolor[HTML]{98D594}} \color[HTML]{000000} 40 & {\cellcolor[HTML]{8DD08A}} \color[HTML]{000000} 43 & {\cellcolor[HTML]{83CB82}} \color[HTML]{000000} 46 & {\cellcolor[HTML]{73C476}} \color[HTML]{000000} 50 & {\cellcolor[HTML]{D3EECD}} \color[HTML]{000000} 20 & {\cellcolor[HTML]{D1EDCB}} \color[HTML]{000000} 21 & {\cellcolor[HTML]{CEECC8}} \color[HTML]{000000} 22 & {\cellcolor[HTML]{CCEBC6}} \color[HTML]{000000} 23 & {\cellcolor[HTML]{CAEAC3}} \color[HTML]{000000} 24 & {\cellcolor[HTML]{C7E9C0}} \color[HTML]{000000} 25 & \bfseries {\cellcolor[HTML]{DFF3DA}} \color[HTML]{000000} 15 & \bfseries {\cellcolor[HTML]{DDF2D8}} \color[HTML]{000000} 16 & {\cellcolor[HTML]{DDF2D8}} \color[HTML]{000000} 16 & \bfseries {\cellcolor[HTML]{DBF1D5}} \color[HTML]{000000} 17 & {\cellcolor[HTML]{DBF1D5}} \color[HTML]{000000} 17 & {\cellcolor[HTML]{D8F0D2}} \color[HTML]{000000} 18 & {\cellcolor[HTML]{CCEBC6}} \color[HTML]{000000} 23 & {\cellcolor[HTML]{C4E8BD}} \color[HTML]{000000} 26 & {\cellcolor[HTML]{BEE5B8}} \color[HTML]{000000} 28 & {\cellcolor[HTML]{B5E1AE}} \color[HTML]{000000} 31 & {\cellcolor[HTML]{ABDDA5}} \color[HTML]{000000} 34 & {\cellcolor[HTML]{A3DA9D}} \color[HTML]{000000} 37 & {\cellcolor[HTML]{91D28E}} \color[HTML]{000000} 42 & {\cellcolor[HTML]{86CC85}} \color[HTML]{000000} 45 & {\cellcolor[HTML]{73C476}} \color[HTML]{000000} 50 & {\cellcolor[HTML]{63BC6E}} \color[HTML]{F1F1F1} 54 & {\cellcolor[HTML]{53B466}} \color[HTML]{F1F1F1} 58 & {\cellcolor[HTML]{43AC5E}} \color[HTML]{F1F1F1} 62 & {\cellcolor[HTML]{D8F0D2}} \color[HTML]{000000} 18 & {\cellcolor[HTML]{D1EDCB}} \color[HTML]{000000} 21 & {\cellcolor[HTML]{C7E9C0}} \color[HTML]{000000} 25 & {\cellcolor[HTML]{BEE5B8}} \color[HTML]{000000} 28 & {\cellcolor[HTML]{B2E0AC}} \color[HTML]{000000} 32 & {\cellcolor[HTML]{A5DB9F}} \color[HTML]{000000} 36 & {\cellcolor[HTML]{98D594}} \color[HTML]{000000} 40 & \bfseries {\cellcolor[HTML]{4BB062}} \color[HTML]{F1F1F1} 60 & \bfseries {\cellcolor[HTML]{39A257}} \color[HTML]{F1F1F1} 66 & \bfseries {\cellcolor[HTML]{2A924A}} \color[HTML]{F1F1F1} 72 & \bfseries {\cellcolor[HTML]{1D8640}} \color[HTML]{F1F1F1} 77 & \bfseries {\cellcolor[HTML]{157F3B}} \color[HTML]{F1F1F1} 80 & \bfseries {\cellcolor[HTML]{107A37}} \color[HTML]{F1F1F1} 82 \\
\end{tabular}



==> export/table_f-rh.tex <==

\begin{tabular}{lm{\colwidth}m{\colwidth}m{\colwidth}m{\colwidth}m{\colwidth}m{\colwidth}m{\colwidth}m{\colwidth}m{\colwidth}m{\colwidth}m{\colwidth}m{\colwidth}m{\colwidth}m{\colwidth}m{\colwidth}m{\colwidth}m{\colwidth}m{\colwidth}m{\colwidth}m{\colwidth}m{\colwidth}m{\colwidth}m{\colwidth}m{\colwidth}m{\colwidth}m{\colwidth}m{\colwidth}m{\colwidth}m{\colwidth}m{\colwidth}m{\colwidth}m{\colwidth}m{\colwidth}m{\colwidth}m{\colwidth}m{\colwidth}m{\colwidth}m{\colwidth}m{\colwidth}m{\colwidth}m{\colwidth}m{\colwidth}m{\colwidth}m{\colwidth}m{\colwidth}m{\colwidth}m{\colwidth}m{\colwidth}m{\colwidth}}
\textbf{Test dataset} & \multicolumn{5}{l}{{\cellcolor[rgb]{.9,.9,.9}} AlexMI} & \multicolumn{6}{l}{BNCI2014001} & \multicolumn{7}{l}{{\cellcolor[rgb]{.9,.9,.9}} BNCI2015001} & \multicolumn{6}{l}{BNCI2015004} & \multicolumn{5}{l}{{\cellcolor[rgb]{.9,.9,.9}} PhysionetMI(I)} & \multicolumn{7}{l}{Schirrmeister2017} & \multicolumn{7}{l}{{\cellcolor[rgb]{.9,.9,.9}} Weibo2014} & \multicolumn{6}{l}{Zhou2016} \\
\textbf{Trials/class} & {\cellcolor[rgb]{.9,.9,.9}} 1 & 2 & {\cellcolor[rgb]{.9,.9,.9}} 4 & 8 & {\cellcolor[rgb]{.9,.9,.9}} 16 & 1 & {\cellcolor[rgb]{.9,.9,.9}} 2 & 4 & {\cellcolor[rgb]{.9,.9,.9}} 8 & 16 & {\cellcolor[rgb]{.9,.9,.9}} 32 & 1 & {\cellcolor[rgb]{.9,.9,.9}} 2 & 4 & {\cellcolor[rgb]{.9,.9,.9}} 8 & 16 & {\cellcolor[rgb]{.9,.9,.9}} 32 & 64 & {\cellcolor[rgb]{.9,.9,.9}} 1 & 2 & {\cellcolor[rgb]{.9,.9,.9}} 4 & 8 & {\cellcolor[rgb]{.9,.9,.9}} 16 & 32 & {\cellcolor[rgb]{.9,.9,.9}} 1 & 2 & {\cellcolor[rgb]{.9,.9,.9}} 4 & 8 & {\cellcolor[rgb]{.9,.9,.9}} 16 & 1 & {\cellcolor[rgb]{.9,.9,.9}} 2 & 4 & {\cellcolor[rgb]{.9,.9,.9}} 8 & 16 & {\cellcolor[rgb]{.9,.9,.9}} 32 & 64 & {\cellcolor[rgb]{.9,.9,.9}} 1 & 2 & {\cellcolor[rgb]{.9,.9,.9}} 4 & 8 & {\cellcolor[rgb]{.9,.9,.9}} 16 & 32 & {\cellcolor[rgb]{.9,.9,.9}} 64 & 1 & {\cellcolor[rgb]{.9,.9,.9}} 2 & 4 & {\cellcolor[rgb]{.9,.9,.9}} 8 & 16 & {\cellcolor[rgb]{.9,.9,.9}} 32 \\
\textbf{Pretraining dataset} & {\cellcolor[rgb]{.9,.9,.9}} & & {\cellcolor[rgb]{.9,.9,.9}} & & {\cellcolor[rgb]{.9,.9,.9}} & & {\cellcolor[rgb]{.9,.9,.9}} & & {\cellcolor[rgb]{.9,.9,.9}} & & {\cellcolor[rgb]{.9,.9,.9}} & & {\cellcolor[rgb]{.9,.9,.9}} & & {\cellcolor[rgb]{.9,.9,.9}} & & {\cellcolor[rgb]{.9,.9,.9}} & & {\cellcolor[rgb]{.9,.9,.9}} & & {\cellcolor[rgb]{.9,.9,.9}} & & {\cellcolor[rgb]{.9,.9,.9}} & & {\cellcolor[rgb]{.9,.9,.9}} & & {\cellcolor[rgb]{.9,.9,.9}} & & {\cellcolor[rgb]{.9,.9,.9}} & & {\cellcolor[rgb]{.9,.9,.9}} & & {\cellcolor[rgb]{.9,.9,.9}} & & {\cellcolor[rgb]{.9,.9,.9}} & & {\cellcolor[rgb]{.9,.9,.9}} & & {\cellcolor[rgb]{.9,.9,.9}} & & {\cellcolor[rgb]{.9,.9,.9}} & & {\cellcolor[rgb]{.9,.9,.9}} & & {\cellcolor[rgb]{.9,.9,.9}} & & {\cellcolor[rgb]{.9,.9,.9}} & & {\cellcolor[rgb]{.9,.9,.9}} \\
{\cellcolor[rgb]{.9,.9,.9}} AlexMI & {\cellcolor[HTML]{D8E7F5}} \color[HTML]{000000} 58 & {\cellcolor[HTML]{DCE9F6}} \color[HTML]{000000} 57 & {\cellcolor[HTML]{DFECF7}} \color[HTML]{000000} 56 & {\cellcolor[HTML]{D0E1F2}} \color[HTML]{000000} 60 & {\cellcolor[HTML]{C3DAEE}} \color[HTML]{000000} 63 & {\cellcolor[HTML]{E3EEF9}} \color[HTML]{000000} 55 & {\cellcolor[HTML]{DCE9F6}} \color[HTML]{000000} 57 & {\cellcolor[HTML]{D0E1F2}} \color[HTML]{000000} 60 & {\cellcolor[HTML]{C8DCF0}} \color[HTML]{000000} 62 & {\cellcolor[HTML]{B0D2E7}} \color[HTML]{000000} 66 & {\cellcolor[HTML]{8CC0DD}} \color[HTML]{000000} 71 & {\cellcolor[HTML]{F3F8FE}} \color[HTML]{000000} 51 & {\cellcolor[HTML]{EFF6FC}} \color[HTML]{000000} 52 & {\cellcolor[HTML]{E7F1FA}} \color[HTML]{000000} 54 & {\cellcolor[HTML]{DFECF7}} \color[HTML]{000000} 56 & {\cellcolor[HTML]{DCE9F6}} \color[HTML]{000000} 57 & {\cellcolor[HTML]{D0E1F2}} \color[HTML]{000000} 60 & {\cellcolor[HTML]{BDD7EC}} \color[HTML]{000000} 64 & {\cellcolor[HTML]{F3F8FE}} \color[HTML]{000000} 51 & {\cellcolor[HTML]{F3F8FE}} \color[HTML]{000000} 51 & {\cellcolor[HTML]{F3F8FE}} \color[HTML]{000000} 51 & {\cellcolor[HTML]{F3F8FE}} \color[HTML]{000000} 51 & {\cellcolor[HTML]{F3F8FE}} \color[HTML]{000000} 51 & {\cellcolor[HTML]{F7FBFF}} \color[HTML]{000000} 50 & {\cellcolor[HTML]{F3F8FE}} \color[HTML]{000000} 51 & {\cellcolor[HTML]{EBF3FB}} \color[HTML]{000000} 53 & {\cellcolor[HTML]{E7F1FA}} \color[HTML]{000000} 54 & {\cellcolor[HTML]{DFECF7}} \color[HTML]{000000} 56 & {\cellcolor[HTML]{D0E1F2}} \color[HTML]{000000} 60 & {\cellcolor[HTML]{C8DCF0}} \color[HTML]{000000} 62 & {\cellcolor[HTML]{A9CFE5}} \color[HTML]{000000} 67 & {\cellcolor[HTML]{84BCDB}} \color[HTML]{000000} 72 & {\cellcolor[HTML]{5DA5D1}} \color[HTML]{F1F1F1} 77 & {\cellcolor[HTML]{4493C7}} \color[HTML]{F1F1F1} 81 & {\cellcolor[HTML]{3383BE}} \color[HTML]{F1F1F1} 84 & {\cellcolor[HTML]{2979B9}} \color[HTML]{F1F1F1} 86 & {\cellcolor[HTML]{F3F8FE}} \color[HTML]{000000} 51 & {\cellcolor[HTML]{F3F8FE}} \color[HTML]{000000} 51 & {\cellcolor[HTML]{F3F8FE}} \color[HTML]{000000} 51 & {\cellcolor[HTML]{EFF6FC}} \color[HTML]{000000} 52 & {\cellcolor[HTML]{E7F1FA}} \color[HTML]{000000} 54 & {\cellcolor[HTML]{DCE9F6}} \color[HTML]{000000} 57 & {\cellcolor[HTML]{CCDFF1}} \color[HTML]{000000} 61 & {\cellcolor[HTML]{F3F8FE}} \color[HTML]{000000} 51 & {\cellcolor[HTML]{E3EEF9}} \color[HTML]{000000} 55 & {\cellcolor[HTML]{DFECF7}} \color[HTML]{000000} 56 & {\cellcolor[HTML]{D8E7F5}} \color[HTML]{000000} 58 & {\cellcolor[HTML]{D0E1F2}} \color[HTML]{000000} 60 & {\cellcolor[HTML]{B7D4EA}} \color[HTML]{000000} 65 \\
BNCI2014001 & {\cellcolor[HTML]{C8DCF0}} \color[HTML]{000000} 62 & {\cellcolor[HTML]{C8DCF0}} \color[HTML]{000000} 62 & {\cellcolor[HTML]{B0D2E7}} \color[HTML]{000000} 66 & {\cellcolor[HTML]{94C4DF}} \color[HTML]{000000} 70 & {\cellcolor[HTML]{7CB7DA}} \color[HTML]{000000} 73 & \bfseries {\cellcolor[HTML]{A9CFE5}} \color[HTML]{000000} 67 & \bfseries {\cellcolor[HTML]{84BCDB}} \color[HTML]{000000} 72 & \bfseries {\cellcolor[HTML]{5DA5D1}} \color[HTML]{F1F1F1} 77 & \bfseries {\cellcolor[HTML]{3E8EC4}} \color[HTML]{F1F1F1} 82 & \bfseries {\cellcolor[HTML]{2E7EBC}} \color[HTML]{F1F1F1} 85 & \bfseries {\cellcolor[HTML]{1F6EB3}} \color[HTML]{F1F1F1} 88 & {\cellcolor[HTML]{D8E7F5}} \color[HTML]{000000} 58 & {\cellcolor[HTML]{CCDFF1}} \color[HTML]{000000} 61 & {\cellcolor[HTML]{BDD7EC}} \color[HTML]{000000} 64 & {\cellcolor[HTML]{A3CCE3}} \color[HTML]{000000} 68 & {\cellcolor[HTML]{8CC0DD}} \color[HTML]{000000} 71 & {\cellcolor[HTML]{74B3D8}} \color[HTML]{000000} 74 & {\cellcolor[HTML]{57A0CE}} \color[HTML]{F1F1F1} 78 & {\cellcolor[HTML]{F7FBFF}} \color[HTML]{000000} 50 & {\cellcolor[HTML]{F7FBFF}} \color[HTML]{000000} 50 & {\cellcolor[HTML]{F3F8FE}} \color[HTML]{000000} 51 & {\cellcolor[HTML]{EFF6FC}} \color[HTML]{000000} 52 & {\cellcolor[HTML]{EBF3FB}} \color[HTML]{000000} 53 & {\cellcolor[HTML]{E7F1FA}} \color[HTML]{000000} 54 & {\cellcolor[HTML]{E3EEF9}} \color[HTML]{000000} 55 & {\cellcolor[HTML]{D8E7F5}} \color[HTML]{000000} 58 & {\cellcolor[HTML]{CCDFF1}} \color[HTML]{000000} 61 & {\cellcolor[HTML]{BDD7EC}} \color[HTML]{000000} 64 & {\cellcolor[HTML]{A9CFE5}} \color[HTML]{000000} 67 & {\cellcolor[HTML]{5DA5D1}} \color[HTML]{F1F1F1} 77 & {\cellcolor[HTML]{3E8EC4}} \color[HTML]{F1F1F1} 82 & {\cellcolor[HTML]{2373B6}} \color[HTML]{F1F1F1} 87 & {\cellcolor[HTML]{1764AB}} \color[HTML]{F1F1F1} 90 & {\cellcolor[HTML]{0E59A2}} \color[HTML]{F1F1F1} 92 & {\cellcolor[HTML]{0A549E}} \color[HTML]{F1F1F1} 93 & {\cellcolor[HTML]{084A91}} \color[HTML]{F1F1F1} 95 & {\cellcolor[HTML]{E3EEF9}} \color[HTML]{000000} 55 & {\cellcolor[HTML]{DFECF7}} \color[HTML]{000000} 56 & {\cellcolor[HTML]{CCDFF1}} \color[HTML]{000000} 61 & {\cellcolor[HTML]{A9CFE5}} \color[HTML]{000000} 67 & {\cellcolor[HTML]{84BCDB}} \color[HTML]{000000} 72 & {\cellcolor[HTML]{57A0CE}} \color[HTML]{F1F1F1} 78 & {\cellcolor[HTML]{4493C7}} \color[HTML]{F1F1F1} 81 & {\cellcolor[HTML]{7CB7DA}} \color[HTML]{000000} 73 & {\cellcolor[HTML]{519CCC}} \color[HTML]{F1F1F1} 79 & {\cellcolor[HTML]{3383BE}} \color[HTML]{F1F1F1} 84 & {\cellcolor[HTML]{2373B6}} \color[HTML]{F1F1F1} 87 & {\cellcolor[HTML]{1B69AF}} \color[HTML]{F1F1F1} 89 & {\cellcolor[HTML]{135FA7}} \color[HTML]{F1F1F1} 91 \\
{\cellcolor[rgb]{.9,.9,.9}} BNCI2014004 & {\cellcolor[HTML]{D0E1F2}} \color[HTML]{000000} 60 & {\cellcolor[HTML]{BDD7EC}} \color[HTML]{000000} 64 & {\cellcolor[HTML]{A9CFE5}} \color[HTML]{000000} 67 & {\cellcolor[HTML]{94C4DF}} \color[HTML]{000000} 70 & {\cellcolor[HTML]{84BCDB}} \color[HTML]{000000} 72 & {\cellcolor[HTML]{DFECF7}} \color[HTML]{000000} 56 & {\cellcolor[HTML]{D3E4F3}} \color[HTML]{000000} 59 & {\cellcolor[HTML]{C8DCF0}} \color[HTML]{000000} 62 & {\cellcolor[HTML]{B0D2E7}} \color[HTML]{000000} 66 & {\cellcolor[HTML]{94C4DF}} \color[HTML]{000000} 70 & {\cellcolor[HTML]{84BCDB}} \color[HTML]{000000} 72 & {\cellcolor[HTML]{D8E7F5}} \color[HTML]{000000} 58 & {\cellcolor[HTML]{D0E1F2}} \color[HTML]{000000} 60 & {\cellcolor[HTML]{C8DCF0}} \color[HTML]{000000} 62 & {\cellcolor[HTML]{B7D4EA}} \color[HTML]{000000} 65 & {\cellcolor[HTML]{A9CFE5}} \color[HTML]{000000} 67 & {\cellcolor[HTML]{94C4DF}} \color[HTML]{000000} 70 & {\cellcolor[HTML]{7CB7DA}} \color[HTML]{000000} 73 & {\cellcolor[HTML]{F3F8FE}} \color[HTML]{000000} 51 & \bfseries {\cellcolor[HTML]{EFF6FC}} \color[HTML]{000000} 52 & \bfseries {\cellcolor[HTML]{EBF3FB}} \color[HTML]{000000} 53 & \bfseries {\cellcolor[HTML]{E7F1FA}} \color[HTML]{000000} 54 & {\cellcolor[HTML]{E3EEF9}} \color[HTML]{000000} 55 & {\cellcolor[HTML]{E7F1FA}} \color[HTML]{000000} 54 & {\cellcolor[HTML]{EBF3FB}} \color[HTML]{000000} 53 & {\cellcolor[HTML]{E7F1FA}} \color[HTML]{000000} 54 & {\cellcolor[HTML]{DCE9F6}} \color[HTML]{000000} 57 & {\cellcolor[HTML]{D0E1F2}} \color[HTML]{000000} 60 & {\cellcolor[HTML]{C3DAEE}} \color[HTML]{000000} 63 & {\cellcolor[HTML]{8CC0DD}} \color[HTML]{000000} 71 & {\cellcolor[HTML]{64A9D3}} \color[HTML]{F1F1F1} 76 & {\cellcolor[HTML]{4A98C9}} \color[HTML]{F1F1F1} 80 & {\cellcolor[HTML]{3383BE}} \color[HTML]{F1F1F1} 84 & {\cellcolor[HTML]{2979B9}} \color[HTML]{F1F1F1} 86 & {\cellcolor[HTML]{1B69AF}} \color[HTML]{F1F1F1} 89 & {\cellcolor[HTML]{135FA7}} \color[HTML]{F1F1F1} 91 & {\cellcolor[HTML]{DCE9F6}} \color[HTML]{000000} 57 & {\cellcolor[HTML]{D8E7F5}} \color[HTML]{000000} 58 & {\cellcolor[HTML]{CCDFF1}} \color[HTML]{000000} 61 & {\cellcolor[HTML]{B0D2E7}} \color[HTML]{000000} 66 & {\cellcolor[HTML]{8CC0DD}} \color[HTML]{000000} 71 & {\cellcolor[HTML]{6AAED6}} \color[HTML]{F1F1F1} 75 & {\cellcolor[HTML]{519CCC}} \color[HTML]{F1F1F1} 79 & {\cellcolor[HTML]{B0D2E7}} \color[HTML]{000000} 66 & {\cellcolor[HTML]{7CB7DA}} \color[HTML]{000000} 73 & {\cellcolor[HTML]{5DA5D1}} \color[HTML]{F1F1F1} 77 & {\cellcolor[HTML]{4493C7}} \color[HTML]{F1F1F1} 81 & {\cellcolor[HTML]{2E7EBC}} \color[HTML]{F1F1F1} 85 & {\cellcolor[HTML]{2373B6}} \color[HTML]{F1F1F1} 87 \\
BNCI2015001 & \bfseries {\cellcolor[HTML]{B7D4EA}} \color[HTML]{000000} 65 & {\cellcolor[HTML]{A9CFE5}} \color[HTML]{000000} 67 & {\cellcolor[HTML]{94C4DF}} \color[HTML]{000000} 70 & {\cellcolor[HTML]{94C4DF}} \color[HTML]{000000} 70 & {\cellcolor[HTML]{94C4DF}} \color[HTML]{000000} 70 & {\cellcolor[HTML]{B7D4EA}} \color[HTML]{000000} 65 & {\cellcolor[HTML]{A3CCE3}} \color[HTML]{000000} 68 & {\cellcolor[HTML]{8CC0DD}} \color[HTML]{000000} 71 & {\cellcolor[HTML]{74B3D8}} \color[HTML]{000000} 74 & {\cellcolor[HTML]{5DA5D1}} \color[HTML]{F1F1F1} 77 & {\cellcolor[HTML]{4A98C9}} \color[HTML]{F1F1F1} 80 & \bfseries {\cellcolor[HTML]{B7D4EA}} \color[HTML]{000000} 65 & \bfseries {\cellcolor[HTML]{9CC9E1}} \color[HTML]{000000} 69 & \bfseries {\cellcolor[HTML]{7CB7DA}} \color[HTML]{000000} 73 & \bfseries {\cellcolor[HTML]{64A9D3}} \color[HTML]{F1F1F1} 76 & \bfseries {\cellcolor[HTML]{519CCC}} \color[HTML]{F1F1F1} 79 & \bfseries {\cellcolor[HTML]{3E8EC4}} \color[HTML]{F1F1F1} 82 & \bfseries {\cellcolor[HTML]{3383BE}} \color[HTML]{F1F1F1} 84 & {\cellcolor[HTML]{F3F8FE}} \color[HTML]{000000} 51 & {\cellcolor[HTML]{F3F8FE}} \color[HTML]{000000} 51 & \bfseries {\cellcolor[HTML]{EBF3FB}} \color[HTML]{000000} 53 & {\cellcolor[HTML]{EBF3FB}} \color[HTML]{000000} 53 & {\cellcolor[HTML]{EBF3FB}} \color[HTML]{000000} 53 & {\cellcolor[HTML]{DFECF7}} \color[HTML]{000000} 56 & \bfseries {\cellcolor[HTML]{D3E4F3}} \color[HTML]{000000} 59 & {\cellcolor[HTML]{D0E1F2}} \color[HTML]{000000} 60 & {\cellcolor[HTML]{C8DCF0}} \color[HTML]{000000} 62 & {\cellcolor[HTML]{BDD7EC}} \color[HTML]{000000} 64 & {\cellcolor[HTML]{A9CFE5}} \color[HTML]{000000} 67 & {\cellcolor[HTML]{64A9D3}} \color[HTML]{F1F1F1} 76 & {\cellcolor[HTML]{3E8EC4}} \color[HTML]{F1F1F1} 82 & {\cellcolor[HTML]{2979B9}} \color[HTML]{F1F1F1} 86 & {\cellcolor[HTML]{1B69AF}} \color[HTML]{F1F1F1} 89 & {\cellcolor[HTML]{1764AB}} \color[HTML]{F1F1F1} 90 & {\cellcolor[HTML]{0E59A2}} \color[HTML]{F1F1F1} 92 & {\cellcolor[HTML]{0A549E}} \color[HTML]{F1F1F1} 93 & \bfseries {\cellcolor[HTML]{BDD7EC}} \color[HTML]{000000} 64 & \bfseries {\cellcolor[HTML]{A9CFE5}} \color[HTML]{000000} 67 & \bfseries {\cellcolor[HTML]{7CB7DA}} \color[HTML]{000000} 73 & \bfseries {\cellcolor[HTML]{5DA5D1}} \color[HTML]{F1F1F1} 77 & \bfseries {\cellcolor[HTML]{4A98C9}} \color[HTML]{F1F1F1} 80 & \bfseries {\cellcolor[HTML]{3E8EC4}} \color[HTML]{F1F1F1} 82 & {\cellcolor[HTML]{3383BE}} \color[HTML]{F1F1F1} 84 & {\cellcolor[HTML]{519CCC}} \color[HTML]{F1F1F1} 79 & {\cellcolor[HTML]{3989C1}} \color[HTML]{F1F1F1} 83 & {\cellcolor[HTML]{2E7EBC}} \color[HTML]{F1F1F1} 85 & {\cellcolor[HTML]{2373B6}} \color[HTML]{F1F1F1} 87 & {\cellcolor[HTML]{1B69AF}} \color[HTML]{F1F1F1} 89 & {\cellcolor[HTML]{1764AB}} \color[HTML]{F1F1F1} 90 \\
{\cellcolor[rgb]{.9,.9,.9}} BNCI2015004 & {\cellcolor[HTML]{F7FBFF}} \color[HTML]{000000} 50 & {\cellcolor[HTML]{F7FBFF}} \color[HTML]{000000} 50 & {\cellcolor[HTML]{F3F8FE}} \color[HTML]{000000} 51 & {\cellcolor[HTML]{F7FBFF}} \color[HTML]{000000} 50 & {\cellcolor[HTML]{EFF6FC}} \color[HTML]{000000} 52 & {\cellcolor[HTML]{EBF3FB}} \color[HTML]{000000} 53 & {\cellcolor[HTML]{E3EEF9}} \color[HTML]{000000} 55 & {\cellcolor[HTML]{DCE9F6}} \color[HTML]{000000} 57 & {\cellcolor[HTML]{CCDFF1}} \color[HTML]{000000} 61 & {\cellcolor[HTML]{B7D4EA}} \color[HTML]{000000} 65 & {\cellcolor[HTML]{9CC9E1}} \color[HTML]{000000} 69 & {\cellcolor[HTML]{EFF6FC}} \color[HTML]{000000} 52 & {\cellcolor[HTML]{EFF6FC}} \color[HTML]{000000} 52 & {\cellcolor[HTML]{EBF3FB}} \color[HTML]{000000} 53 & {\cellcolor[HTML]{E3EEF9}} \color[HTML]{000000} 55 & {\cellcolor[HTML]{DCE9F6}} \color[HTML]{000000} 57 & {\cellcolor[HTML]{D0E1F2}} \color[HTML]{000000} 60 & {\cellcolor[HTML]{BDD7EC}} \color[HTML]{000000} 64 & {\cellcolor[HTML]{F7FBFF}} \color[HTML]{000000} 49 & {\cellcolor[HTML]{F7FBFF}} \color[HTML]{000000} 49 & {\cellcolor[HTML]{F7FBFF}} \color[HTML]{000000} 49 & {\cellcolor[HTML]{F7FBFF}} \color[HTML]{000000} 50 & {\cellcolor[HTML]{EFF6FC}} \color[HTML]{000000} 52 & {\cellcolor[HTML]{F3F8FE}} \color[HTML]{000000} 51 & {\cellcolor[HTML]{EFF6FC}} \color[HTML]{000000} 52 & {\cellcolor[HTML]{EFF6FC}} \color[HTML]{000000} 52 & {\cellcolor[HTML]{EBF3FB}} \color[HTML]{000000} 53 & {\cellcolor[HTML]{E7F1FA}} \color[HTML]{000000} 54 & {\cellcolor[HTML]{DFECF7}} \color[HTML]{000000} 56 & {\cellcolor[HTML]{D3E4F3}} \color[HTML]{000000} 59 & {\cellcolor[HTML]{C8DCF0}} \color[HTML]{000000} 62 & {\cellcolor[HTML]{A9CFE5}} \color[HTML]{000000} 67 & {\cellcolor[HTML]{84BCDB}} \color[HTML]{000000} 72 & {\cellcolor[HTML]{64A9D3}} \color[HTML]{F1F1F1} 76 & {\cellcolor[HTML]{4A98C9}} \color[HTML]{F1F1F1} 80 & {\cellcolor[HTML]{3383BE}} \color[HTML]{F1F1F1} 84 & {\cellcolor[HTML]{F7FBFF}} \color[HTML]{000000} 50 & {\cellcolor[HTML]{F3F8FE}} \color[HTML]{000000} 51 & {\cellcolor[HTML]{F3F8FE}} \color[HTML]{000000} 51 & {\cellcolor[HTML]{F3F8FE}} \color[HTML]{000000} 51 & {\cellcolor[HTML]{F3F8FE}} \color[HTML]{000000} 51 & {\cellcolor[HTML]{E3EEF9}} \color[HTML]{000000} 55 & {\cellcolor[HTML]{D8E7F5}} \color[HTML]{000000} 58 & {\cellcolor[HTML]{EFF6FC}} \color[HTML]{000000} 52 & {\cellcolor[HTML]{EBF3FB}} \color[HTML]{000000} 53 & {\cellcolor[HTML]{E3EEF9}} \color[HTML]{000000} 55 & {\cellcolor[HTML]{DCE9F6}} \color[HTML]{000000} 57 & {\cellcolor[HTML]{D0E1F2}} \color[HTML]{000000} 60 & {\cellcolor[HTML]{C3DAEE}} \color[HTML]{000000} 63 \\
Cho2017 & {\cellcolor[HTML]{EBF3FB}} \color[HTML]{000000} 53 & {\cellcolor[HTML]{E7F1FA}} \color[HTML]{000000} 54 & {\cellcolor[HTML]{F3F8FE}} \color[HTML]{000000} 51 & {\cellcolor[HTML]{EFF6FC}} \color[HTML]{000000} 52 & {\cellcolor[HTML]{DFECF7}} \color[HTML]{000000} 56 & {\cellcolor[HTML]{EFF6FC}} \color[HTML]{000000} 52 & {\cellcolor[HTML]{E7F1FA}} \color[HTML]{000000} 54 & {\cellcolor[HTML]{E3EEF9}} \color[HTML]{000000} 55 & {\cellcolor[HTML]{D8E7F5}} \color[HTML]{000000} 58 & {\cellcolor[HTML]{CCDFF1}} \color[HTML]{000000} 61 & {\cellcolor[HTML]{BDD7EC}} \color[HTML]{000000} 64 & {\cellcolor[HTML]{EFF6FC}} \color[HTML]{000000} 52 & {\cellcolor[HTML]{EFF6FC}} \color[HTML]{000000} 52 & {\cellcolor[HTML]{EBF3FB}} \color[HTML]{000000} 53 & {\cellcolor[HTML]{E3EEF9}} \color[HTML]{000000} 55 & {\cellcolor[HTML]{DCE9F6}} \color[HTML]{000000} 57 & {\cellcolor[HTML]{D8E7F5}} \color[HTML]{000000} 58 & {\cellcolor[HTML]{CCDFF1}} \color[HTML]{000000} 61 & {\cellcolor[HTML]{F3F8FE}} \color[HTML]{000000} 51 & {\cellcolor[HTML]{F3F8FE}} \color[HTML]{000000} 51 & {\cellcolor[HTML]{F7FBFF}} \color[HTML]{000000} 50 & {\cellcolor[HTML]{F7FBFF}} \color[HTML]{000000} 50 & {\cellcolor[HTML]{F7FBFF}} \color[HTML]{000000} 49 & {\cellcolor[HTML]{F3F8FE}} \color[HTML]{000000} 51 & {\cellcolor[HTML]{EBF3FB}} \color[HTML]{000000} 53 & {\cellcolor[HTML]{E3EEF9}} \color[HTML]{000000} 55 & {\cellcolor[HTML]{DCE9F6}} \color[HTML]{000000} 57 & {\cellcolor[HTML]{D3E4F3}} \color[HTML]{000000} 59 & {\cellcolor[HTML]{CCDFF1}} \color[HTML]{000000} 61 & {\cellcolor[HTML]{DFECF7}} \color[HTML]{000000} 56 & {\cellcolor[HTML]{D3E4F3}} \color[HTML]{000000} 59 & {\cellcolor[HTML]{C8DCF0}} \color[HTML]{000000} 62 & {\cellcolor[HTML]{B0D2E7}} \color[HTML]{000000} 66 & {\cellcolor[HTML]{94C4DF}} \color[HTML]{000000} 70 & {\cellcolor[HTML]{74B3D8}} \color[HTML]{000000} 74 & {\cellcolor[HTML]{57A0CE}} \color[HTML]{F1F1F1} 78 & {\cellcolor[HTML]{F7FBFF}} \color[HTML]{000000} 50 & {\cellcolor[HTML]{F7FBFF}} \color[HTML]{000000} 50 & {\cellcolor[HTML]{F3F8FE}} \color[HTML]{000000} 51 & {\cellcolor[HTML]{F3F8FE}} \color[HTML]{000000} 51 & {\cellcolor[HTML]{F3F8FE}} \color[HTML]{000000} 51 & {\cellcolor[HTML]{EFF6FC}} \color[HTML]{000000} 52 & {\cellcolor[HTML]{E7F1FA}} \color[HTML]{000000} 54 & {\cellcolor[HTML]{E7F1FA}} \color[HTML]{000000} 54 & {\cellcolor[HTML]{DFECF7}} \color[HTML]{000000} 56 & {\cellcolor[HTML]{D0E1F2}} \color[HTML]{000000} 60 & {\cellcolor[HTML]{C8DCF0}} \color[HTML]{000000} 62 & {\cellcolor[HTML]{B7D4EA}} \color[HTML]{000000} 65 & {\cellcolor[HTML]{A3CCE3}} \color[HTML]{000000} 68 \\
{\cellcolor[rgb]{.9,.9,.9}} Lee2019\_MI & {\cellcolor[HTML]{D3E4F3}} \color[HTML]{000000} 59 & {\cellcolor[HTML]{BDD7EC}} \color[HTML]{000000} 64 & {\cellcolor[HTML]{A3CCE3}} \color[HTML]{000000} 68 & {\cellcolor[HTML]{8CC0DD}} \color[HTML]{000000} 71 & {\cellcolor[HTML]{74B3D8}} \color[HTML]{000000} 74 & {\cellcolor[HTML]{CCDFF1}} \color[HTML]{000000} 61 & {\cellcolor[HTML]{BDD7EC}} \color[HTML]{000000} 64 & {\cellcolor[HTML]{A3CCE3}} \color[HTML]{000000} 68 & {\cellcolor[HTML]{8CC0DD}} \color[HTML]{000000} 71 & {\cellcolor[HTML]{6AAED6}} \color[HTML]{F1F1F1} 75 & {\cellcolor[HTML]{519CCC}} \color[HTML]{F1F1F1} 79 & {\cellcolor[HTML]{D3E4F3}} \color[HTML]{000000} 59 & {\cellcolor[HTML]{C8DCF0}} \color[HTML]{000000} 62 & {\cellcolor[HTML]{B7D4EA}} \color[HTML]{000000} 65 & {\cellcolor[HTML]{A3CCE3}} \color[HTML]{000000} 68 & {\cellcolor[HTML]{8CC0DD}} \color[HTML]{000000} 71 & {\cellcolor[HTML]{6AAED6}} \color[HTML]{F1F1F1} 75 & {\cellcolor[HTML]{519CCC}} \color[HTML]{F1F1F1} 79 & {\cellcolor[HTML]{F3F8FE}} \color[HTML]{000000} 51 & {\cellcolor[HTML]{F7FBFF}} \color[HTML]{000000} 50 & {\cellcolor[HTML]{F7FBFF}} \color[HTML]{000000} 50 & {\cellcolor[HTML]{F3F8FE}} \color[HTML]{000000} 51 & {\cellcolor[HTML]{F3F8FE}} \color[HTML]{000000} 51 & {\cellcolor[HTML]{EBF3FB}} \color[HTML]{000000} 53 & {\cellcolor[HTML]{DCE9F6}} \color[HTML]{000000} 57 & {\cellcolor[HTML]{D0E1F2}} \color[HTML]{000000} 60 & {\cellcolor[HTML]{C3DAEE}} \color[HTML]{000000} 63 & {\cellcolor[HTML]{B0D2E7}} \color[HTML]{000000} 66 & {\cellcolor[HTML]{94C4DF}} \color[HTML]{000000} 70 & {\cellcolor[HTML]{9CC9E1}} \color[HTML]{000000} 69 & {\cellcolor[HTML]{74B3D8}} \color[HTML]{000000} 74 & {\cellcolor[HTML]{519CCC}} \color[HTML]{F1F1F1} 79 & {\cellcolor[HTML]{3383BE}} \color[HTML]{F1F1F1} 84 & {\cellcolor[HTML]{1F6EB3}} \color[HTML]{F1F1F1} 88 & {\cellcolor[HTML]{135FA7}} \color[HTML]{F1F1F1} 91 & {\cellcolor[HTML]{0A549E}} \color[HTML]{F1F1F1} 93 & {\cellcolor[HTML]{D0E1F2}} \color[HTML]{000000} 60 & {\cellcolor[HTML]{B7D4EA}} \color[HTML]{000000} 65 & {\cellcolor[HTML]{94C4DF}} \color[HTML]{000000} 70 & {\cellcolor[HTML]{74B3D8}} \color[HTML]{000000} 74 & {\cellcolor[HTML]{57A0CE}} \color[HTML]{F1F1F1} 78 & {\cellcolor[HTML]{4A98C9}} \color[HTML]{F1F1F1} 80 & {\cellcolor[HTML]{3E8EC4}} \color[HTML]{F1F1F1} 82 & {\cellcolor[HTML]{57A0CE}} \color[HTML]{F1F1F1} 78 & {\cellcolor[HTML]{3E8EC4}} \color[HTML]{F1F1F1} 82 & {\cellcolor[HTML]{2979B9}} \color[HTML]{F1F1F1} 86 & {\cellcolor[HTML]{1F6EB3}} \color[HTML]{F1F1F1} 88 & {\cellcolor[HTML]{1764AB}} \color[HTML]{F1F1F1} 90 & {\cellcolor[HTML]{0E59A2}} \color[HTML]{F1F1F1} 92 \\
Ofner2017(I) & {\cellcolor[HTML]{F7FBFF}} \color[HTML]{000000} 50 & {\cellcolor[HTML]{F7FBFF}} \color[HTML]{000000} 50 & {\cellcolor[HTML]{F7FBFF}} \color[HTML]{000000} 50 & {\cellcolor[HTML]{F7FBFF}} \color[HTML]{000000} 50 & {\cellcolor[HTML]{F7FBFF}} \color[HTML]{000000} 50 & {\cellcolor[HTML]{F7FBFF}} \color[HTML]{000000} 50 & {\cellcolor[HTML]{F7FBFF}} \color[HTML]{000000} 50 & {\cellcolor[HTML]{F7FBFF}} \color[HTML]{000000} 50 & {\cellcolor[HTML]{F7FBFF}} \color[HTML]{000000} 50 & {\cellcolor[HTML]{F7FBFF}} \color[HTML]{000000} 50 & {\cellcolor[HTML]{F7FBFF}} \color[HTML]{000000} 50 & {\cellcolor[HTML]{F7FBFF}} \color[HTML]{000000} 50 & {\cellcolor[HTML]{F7FBFF}} \color[HTML]{000000} 50 & {\cellcolor[HTML]{F7FBFF}} \color[HTML]{000000} 50 & {\cellcolor[HTML]{F7FBFF}} \color[HTML]{000000} 50 & {\cellcolor[HTML]{F7FBFF}} \color[HTML]{000000} 50 & {\cellcolor[HTML]{F7FBFF}} \color[HTML]{000000} 50 & {\cellcolor[HTML]{F7FBFF}} \color[HTML]{000000} 50 & {\cellcolor[HTML]{F7FBFF}} \color[HTML]{000000} 50 & {\cellcolor[HTML]{F7FBFF}} \color[HTML]{000000} 50 & {\cellcolor[HTML]{F7FBFF}} \color[HTML]{000000} 50 & {\cellcolor[HTML]{F7FBFF}} \color[HTML]{000000} 50 & {\cellcolor[HTML]{F7FBFF}} \color[HTML]{000000} 50 & {\cellcolor[HTML]{F7FBFF}} \color[HTML]{000000} 50 & {\cellcolor[HTML]{F7FBFF}} \color[HTML]{000000} 50 & {\cellcolor[HTML]{F7FBFF}} \color[HTML]{000000} 50 & {\cellcolor[HTML]{F7FBFF}} \color[HTML]{000000} 50 & {\cellcolor[HTML]{F7FBFF}} \color[HTML]{000000} 50 & {\cellcolor[HTML]{F7FBFF}} \color[HTML]{000000} 50 & {\cellcolor[HTML]{F7FBFF}} \color[HTML]{000000} 50 & {\cellcolor[HTML]{F7FBFF}} \color[HTML]{000000} 50 & {\cellcolor[HTML]{F7FBFF}} \color[HTML]{000000} 50 & {\cellcolor[HTML]{F7FBFF}} \color[HTML]{000000} 50 & {\cellcolor[HTML]{F7FBFF}} \color[HTML]{000000} 50 & {\cellcolor[HTML]{F7FBFF}} \color[HTML]{000000} 50 & {\cellcolor[HTML]{F7FBFF}} \color[HTML]{000000} 50 & {\cellcolor[HTML]{F7FBFF}} \color[HTML]{000000} 50 & {\cellcolor[HTML]{F7FBFF}} \color[HTML]{000000} 50 & {\cellcolor[HTML]{F7FBFF}} \color[HTML]{000000} 50 & {\cellcolor[HTML]{F7FBFF}} \color[HTML]{000000} 50 & {\cellcolor[HTML]{F7FBFF}} \color[HTML]{000000} 50 & {\cellcolor[HTML]{F7FBFF}} \color[HTML]{000000} 50 & {\cellcolor[HTML]{F7FBFF}} \color[HTML]{000000} 50 & {\cellcolor[HTML]{F7FBFF}} \color[HTML]{000000} 50 & {\cellcolor[HTML]{F7FBFF}} \color[HTML]{000000} 50 & {\cellcolor[HTML]{F7FBFF}} \color[HTML]{000000} 50 & {\cellcolor[HTML]{F7FBFF}} \color[HTML]{000000} 50 & {\cellcolor[HTML]{F7FBFF}} \color[HTML]{000000} 50 & {\cellcolor[HTML]{F7FBFF}} \color[HTML]{000000} 50 \\
{\cellcolor[rgb]{.9,.9,.9}} PhysionetMI(I,E) & {\cellcolor[HTML]{BDD7EC}} \color[HTML]{000000} 64 & \bfseries {\cellcolor[HTML]{A3CCE3}} \color[HTML]{000000} 68 & {\cellcolor[HTML]{A3CCE3}} \color[HTML]{000000} 68 & \bfseries {\cellcolor[HTML]{7CB7DA}} \color[HTML]{000000} 73 & \bfseries {\cellcolor[HTML]{57A0CE}} \color[HTML]{F1F1F1} 78 & {\cellcolor[HTML]{B7D4EA}} \color[HTML]{000000} 65 & {\cellcolor[HTML]{9CC9E1}} \color[HTML]{000000} 69 & {\cellcolor[HTML]{7CB7DA}} \color[HTML]{000000} 73 & {\cellcolor[HTML]{57A0CE}} \color[HTML]{F1F1F1} 78 & {\cellcolor[HTML]{3E8EC4}} \color[HTML]{F1F1F1} 82 & {\cellcolor[HTML]{2979B9}} \color[HTML]{F1F1F1} 86 & {\cellcolor[HTML]{CCDFF1}} \color[HTML]{000000} 61 & {\cellcolor[HTML]{C3DAEE}} \color[HTML]{000000} 63 & {\cellcolor[HTML]{A9CFE5}} \color[HTML]{000000} 67 & {\cellcolor[HTML]{94C4DF}} \color[HTML]{000000} 70 & {\cellcolor[HTML]{7CB7DA}} \color[HTML]{000000} 73 & {\cellcolor[HTML]{5DA5D1}} \color[HTML]{F1F1F1} 77 & {\cellcolor[HTML]{4493C7}} \color[HTML]{F1F1F1} 81 & {\cellcolor[HTML]{F7FBFF}} \color[HTML]{000000} 49 & {\cellcolor[HTML]{F7FBFF}} \color[HTML]{000000} 50 & \bfseries {\cellcolor[HTML]{EBF3FB}} \color[HTML]{000000} 53 & {\cellcolor[HTML]{EBF3FB}} \color[HTML]{000000} 53 & \bfseries {\cellcolor[HTML]{DFECF7}} \color[HTML]{000000} 56 & \bfseries {\cellcolor[HTML]{D8E7F5}} \color[HTML]{000000} 58 & {\cellcolor[HTML]{D8E7F5}} \color[HTML]{000000} 58 & \bfseries {\cellcolor[HTML]{C8DCF0}} \color[HTML]{000000} 62 & \bfseries {\cellcolor[HTML]{B0D2E7}} \color[HTML]{000000} 66 & \bfseries {\cellcolor[HTML]{9CC9E1}} \color[HTML]{000000} 69 & \bfseries {\cellcolor[HTML]{8CC0DD}} \color[HTML]{000000} 71 & {\cellcolor[HTML]{57A0CE}} \color[HTML]{F1F1F1} 78 & {\cellcolor[HTML]{3383BE}} \color[HTML]{F1F1F1} 84 & {\cellcolor[HTML]{1F6EB3}} \color[HTML]{F1F1F1} 88 & {\cellcolor[HTML]{1764AB}} \color[HTML]{F1F1F1} 90 & {\cellcolor[HTML]{0E59A2}} \color[HTML]{F1F1F1} 92 & {\cellcolor[HTML]{084F99}} \color[HTML]{F1F1F1} 94 & {\cellcolor[HTML]{084A91}} \color[HTML]{F1F1F1} 95 & {\cellcolor[HTML]{D0E1F2}} \color[HTML]{000000} 60 & {\cellcolor[HTML]{C3DAEE}} \color[HTML]{000000} 63 & {\cellcolor[HTML]{A3CCE3}} \color[HTML]{000000} 68 & {\cellcolor[HTML]{84BCDB}} \color[HTML]{000000} 72 & {\cellcolor[HTML]{5DA5D1}} \color[HTML]{F1F1F1} 77 & \bfseries {\cellcolor[HTML]{3E8EC4}} \color[HTML]{F1F1F1} 82 & \bfseries {\cellcolor[HTML]{2E7EBC}} \color[HTML]{F1F1F1} 85 & {\cellcolor[HTML]{84BCDB}} \color[HTML]{000000} 72 & {\cellcolor[HTML]{5DA5D1}} \color[HTML]{F1F1F1} 77 & {\cellcolor[HTML]{4493C7}} \color[HTML]{F1F1F1} 81 & {\cellcolor[HTML]{2E7EBC}} \color[HTML]{F1F1F1} 85 & {\cellcolor[HTML]{1F6EB3}} \color[HTML]{F1F1F1} 88 & {\cellcolor[HTML]{135FA7}} \color[HTML]{F1F1F1} 91 \\
Schirrmeister2017 & {\cellcolor[HTML]{BDD7EC}} \color[HTML]{000000} 64 & {\cellcolor[HTML]{B0D2E7}} \color[HTML]{000000} 66 & \bfseries {\cellcolor[HTML]{8CC0DD}} \color[HTML]{000000} 71 & {\cellcolor[HTML]{84BCDB}} \color[HTML]{000000} 72 & {\cellcolor[HTML]{74B3D8}} \color[HTML]{000000} 74 & {\cellcolor[HTML]{CCDFF1}} \color[HTML]{000000} 61 & {\cellcolor[HTML]{BDD7EC}} \color[HTML]{000000} 64 & {\cellcolor[HTML]{94C4DF}} \color[HTML]{000000} 70 & {\cellcolor[HTML]{6AAED6}} \color[HTML]{F1F1F1} 75 & {\cellcolor[HTML]{4A98C9}} \color[HTML]{F1F1F1} 80 & {\cellcolor[HTML]{3989C1}} \color[HTML]{F1F1F1} 83 & {\cellcolor[HTML]{BDD7EC}} \color[HTML]{000000} 64 & {\cellcolor[HTML]{B0D2E7}} \color[HTML]{000000} 66 & {\cellcolor[HTML]{A3CCE3}} \color[HTML]{000000} 68 & {\cellcolor[HTML]{8CC0DD}} \color[HTML]{000000} 71 & {\cellcolor[HTML]{6AAED6}} \color[HTML]{F1F1F1} 75 & {\cellcolor[HTML]{5DA5D1}} \color[HTML]{F1F1F1} 77 & {\cellcolor[HTML]{4A98C9}} \color[HTML]{F1F1F1} 80 & {\cellcolor[HTML]{F7FBFF}} \color[HTML]{000000} 48 & {\cellcolor[HTML]{F7FBFF}} \color[HTML]{000000} 49 & {\cellcolor[HTML]{F7FBFF}} \color[HTML]{000000} 49 & {\cellcolor[HTML]{F7FBFF}} \color[HTML]{000000} 50 & {\cellcolor[HTML]{F3F8FE}} \color[HTML]{000000} 51 & {\cellcolor[HTML]{EFF6FC}} \color[HTML]{000000} 52 & {\cellcolor[HTML]{DFECF7}} \color[HTML]{000000} 56 & {\cellcolor[HTML]{D8E7F5}} \color[HTML]{000000} 58 & {\cellcolor[HTML]{CCDFF1}} \color[HTML]{000000} 61 & {\cellcolor[HTML]{BDD7EC}} \color[HTML]{000000} 64 & {\cellcolor[HTML]{A9CFE5}} \color[HTML]{000000} 67 & \bfseries {\cellcolor[HTML]{3383BE}} \color[HTML]{F1F1F1} 84 & \bfseries {\cellcolor[HTML]{1B69AF}} \color[HTML]{F1F1F1} 89 & \bfseries {\cellcolor[HTML]{0E59A2}} \color[HTML]{F1F1F1} 92 & \bfseries {\cellcolor[HTML]{084F99}} \color[HTML]{F1F1F1} 94 & \bfseries {\cellcolor[HTML]{08458A}} \color[HTML]{F1F1F1} 96 & \bfseries {\cellcolor[HTML]{084082}} \color[HTML]{F1F1F1} 97 & \bfseries {\cellcolor[HTML]{084082}} \color[HTML]{F1F1F1} 97 & {\cellcolor[HTML]{D3E4F3}} \color[HTML]{000000} 59 & {\cellcolor[HTML]{C3DAEE}} \color[HTML]{000000} 63 & {\cellcolor[HTML]{A3CCE3}} \color[HTML]{000000} 68 & {\cellcolor[HTML]{7CB7DA}} \color[HTML]{000000} 73 & {\cellcolor[HTML]{5DA5D1}} \color[HTML]{F1F1F1} 77 & {\cellcolor[HTML]{4493C7}} \color[HTML]{F1F1F1} 81 & {\cellcolor[HTML]{3383BE}} \color[HTML]{F1F1F1} 84 & {\cellcolor[HTML]{6AAED6}} \color[HTML]{F1F1F1} 75 & {\cellcolor[HTML]{4A98C9}} \color[HTML]{F1F1F1} 80 & {\cellcolor[HTML]{3383BE}} \color[HTML]{F1F1F1} 84 & {\cellcolor[HTML]{1F6EB3}} \color[HTML]{F1F1F1} 88 & {\cellcolor[HTML]{135FA7}} \color[HTML]{F1F1F1} 91 & {\cellcolor[HTML]{0E59A2}} \color[HTML]{F1F1F1} 92 \\
{\cellcolor[rgb]{.9,.9,.9}} Weibo2014 & {\cellcolor[HTML]{BDD7EC}} \color[HTML]{000000} 64 & {\cellcolor[HTML]{B7D4EA}} \color[HTML]{000000} 65 & {\cellcolor[HTML]{9CC9E1}} \color[HTML]{000000} 69 & {\cellcolor[HTML]{8CC0DD}} \color[HTML]{000000} 71 & {\cellcolor[HTML]{8CC0DD}} \color[HTML]{000000} 71 & {\cellcolor[HTML]{CCDFF1}} \color[HTML]{000000} 61 & {\cellcolor[HTML]{BDD7EC}} \color[HTML]{000000} 64 & {\cellcolor[HTML]{A3CCE3}} \color[HTML]{000000} 68 & {\cellcolor[HTML]{7CB7DA}} \color[HTML]{000000} 73 & {\cellcolor[HTML]{57A0CE}} \color[HTML]{F1F1F1} 78 & {\cellcolor[HTML]{3E8EC4}} \color[HTML]{F1F1F1} 82 & {\cellcolor[HTML]{D8E7F5}} \color[HTML]{000000} 58 & {\cellcolor[HTML]{CCDFF1}} \color[HTML]{000000} 61 & {\cellcolor[HTML]{C3DAEE}} \color[HTML]{000000} 63 & {\cellcolor[HTML]{B7D4EA}} \color[HTML]{000000} 65 & {\cellcolor[HTML]{9CC9E1}} \color[HTML]{000000} 69 & {\cellcolor[HTML]{84BCDB}} \color[HTML]{000000} 72 & {\cellcolor[HTML]{64A9D3}} \color[HTML]{F1F1F1} 76 & \bfseries {\cellcolor[HTML]{EFF6FC}} \color[HTML]{000000} 52 & {\cellcolor[HTML]{F3F8FE}} \color[HTML]{000000} 51 & {\cellcolor[HTML]{EFF6FC}} \color[HTML]{000000} 52 & \bfseries {\cellcolor[HTML]{E7F1FA}} \color[HTML]{000000} 54 & {\cellcolor[HTML]{E7F1FA}} \color[HTML]{000000} 54 & {\cellcolor[HTML]{E7F1FA}} \color[HTML]{000000} 54 & {\cellcolor[HTML]{DFECF7}} \color[HTML]{000000} 56 & {\cellcolor[HTML]{D3E4F3}} \color[HTML]{000000} 59 & {\cellcolor[HTML]{CCDFF1}} \color[HTML]{000000} 61 & {\cellcolor[HTML]{BDD7EC}} \color[HTML]{000000} 64 & {\cellcolor[HTML]{A9CFE5}} \color[HTML]{000000} 67 & {\cellcolor[HTML]{74B3D8}} \color[HTML]{000000} 74 & {\cellcolor[HTML]{519CCC}} \color[HTML]{F1F1F1} 79 & {\cellcolor[HTML]{3989C1}} \color[HTML]{F1F1F1} 83 & {\cellcolor[HTML]{2979B9}} \color[HTML]{F1F1F1} 86 & {\cellcolor[HTML]{1B69AF}} \color[HTML]{F1F1F1} 89 & {\cellcolor[HTML]{135FA7}} \color[HTML]{F1F1F1} 91 & {\cellcolor[HTML]{0E59A2}} \color[HTML]{F1F1F1} 92 & {\cellcolor[HTML]{E7F1FA}} \color[HTML]{000000} 54 & {\cellcolor[HTML]{DFECF7}} \color[HTML]{000000} 56 & {\cellcolor[HTML]{D3E4F3}} \color[HTML]{000000} 59 & {\cellcolor[HTML]{B7D4EA}} \color[HTML]{000000} 65 & {\cellcolor[HTML]{84BCDB}} \color[HTML]{000000} 72 & {\cellcolor[HTML]{5DA5D1}} \color[HTML]{F1F1F1} 77 & {\cellcolor[HTML]{4493C7}} \color[HTML]{F1F1F1} 81 & {\cellcolor[HTML]{7CB7DA}} \color[HTML]{000000} 73 & {\cellcolor[HTML]{64A9D3}} \color[HTML]{F1F1F1} 76 & {\cellcolor[HTML]{57A0CE}} \color[HTML]{F1F1F1} 78 & {\cellcolor[HTML]{4493C7}} \color[HTML]{F1F1F1} 81 & {\cellcolor[HTML]{3989C1}} \color[HTML]{F1F1F1} 83 & {\cellcolor[HTML]{2E7EBC}} \color[HTML]{F1F1F1} 85 \\
Zhou2016 & {\cellcolor[HTML]{D0E1F2}} \color[HTML]{000000} 60 & {\cellcolor[HTML]{BDD7EC}} \color[HTML]{000000} 64 & {\cellcolor[HTML]{A3CCE3}} \color[HTML]{000000} 68 & {\cellcolor[HTML]{A3CCE3}} \color[HTML]{000000} 68 & {\cellcolor[HTML]{8CC0DD}} \color[HTML]{000000} 71 & {\cellcolor[HTML]{CCDFF1}} \color[HTML]{000000} 61 & {\cellcolor[HTML]{BDD7EC}} \color[HTML]{000000} 64 & {\cellcolor[HTML]{A9CFE5}} \color[HTML]{000000} 67 & {\cellcolor[HTML]{8CC0DD}} \color[HTML]{000000} 71 & {\cellcolor[HTML]{6AAED6}} \color[HTML]{F1F1F1} 75 & {\cellcolor[HTML]{519CCC}} \color[HTML]{F1F1F1} 79 & {\cellcolor[HTML]{BDD7EC}} \color[HTML]{000000} 64 & {\cellcolor[HTML]{B0D2E7}} \color[HTML]{000000} 66 & {\cellcolor[HTML]{9CC9E1}} \color[HTML]{000000} 69 & {\cellcolor[HTML]{8CC0DD}} \color[HTML]{000000} 71 & {\cellcolor[HTML]{74B3D8}} \color[HTML]{000000} 74 & {\cellcolor[HTML]{64A9D3}} \color[HTML]{F1F1F1} 76 & {\cellcolor[HTML]{57A0CE}} \color[HTML]{F1F1F1} 78 & {\cellcolor[HTML]{F7FBFF}} \color[HTML]{000000} 49 & {\cellcolor[HTML]{F7FBFF}} \color[HTML]{000000} 50 & {\cellcolor[HTML]{F3F8FE}} \color[HTML]{000000} 51 & {\cellcolor[HTML]{EFF6FC}} \color[HTML]{000000} 52 & {\cellcolor[HTML]{EBF3FB}} \color[HTML]{000000} 53 & {\cellcolor[HTML]{E7F1FA}} \color[HTML]{000000} 54 & {\cellcolor[HTML]{DCE9F6}} \color[HTML]{000000} 57 & {\cellcolor[HTML]{D0E1F2}} \color[HTML]{000000} 60 & {\cellcolor[HTML]{CCDFF1}} \color[HTML]{000000} 61 & {\cellcolor[HTML]{BDD7EC}} \color[HTML]{000000} 64 & {\cellcolor[HTML]{A9CFE5}} \color[HTML]{000000} 67 & {\cellcolor[HTML]{7CB7DA}} \color[HTML]{000000} 73 & {\cellcolor[HTML]{57A0CE}} \color[HTML]{F1F1F1} 78 & {\cellcolor[HTML]{3E8EC4}} \color[HTML]{F1F1F1} 82 & {\cellcolor[HTML]{2979B9}} \color[HTML]{F1F1F1} 86 & {\cellcolor[HTML]{1F6EB3}} \color[HTML]{F1F1F1} 88 & {\cellcolor[HTML]{1764AB}} \color[HTML]{F1F1F1} 90 & {\cellcolor[HTML]{0E59A2}} \color[HTML]{F1F1F1} 92 & {\cellcolor[HTML]{CCDFF1}} \color[HTML]{000000} 61 & {\cellcolor[HTML]{B7D4EA}} \color[HTML]{000000} 65 & {\cellcolor[HTML]{9CC9E1}} \color[HTML]{000000} 69 & {\cellcolor[HTML]{7CB7DA}} \color[HTML]{000000} 73 & {\cellcolor[HTML]{57A0CE}} \color[HTML]{F1F1F1} 78 & {\cellcolor[HTML]{4A98C9}} \color[HTML]{F1F1F1} 80 & {\cellcolor[HTML]{3989C1}} \color[HTML]{F1F1F1} 83 & \bfseries {\cellcolor[HTML]{2E7EBC}} \color[HTML]{F1F1F1} 85 & \bfseries {\cellcolor[HTML]{1B69AF}} \color[HTML]{F1F1F1} 89 & \bfseries {\cellcolor[HTML]{0E59A2}} \color[HTML]{F1F1F1} 92 & \bfseries {\cellcolor[HTML]{084F99}} \color[HTML]{F1F1F1} 94 & \bfseries {\cellcolor[HTML]{084A91}} \color[HTML]{F1F1F1} 95 & \bfseries {\cellcolor[HTML]{08458A}} \color[HTML]{F1F1F1} 96 \\
\end{tabular}



==> export/table_lh-rh.tex <==

\begin{tabular}{lm{\colwidth}m{\colwidth}m{\colwidth}m{\colwidth}m{\colwidth}m{\colwidth}m{\colwidth}m{\colwidth}m{\colwidth}m{\colwidth}m{\colwidth}m{\colwidth}m{\colwidth}m{\colwidth}m{\colwidth}m{\colwidth}m{\colwidth}m{\colwidth}m{\colwidth}m{\colwidth}m{\colwidth}m{\colwidth}m{\colwidth}m{\colwidth}m{\colwidth}m{\colwidth}m{\colwidth}m{\colwidth}m{\colwidth}m{\colwidth}m{\colwidth}m{\colwidth}m{\colwidth}m{\colwidth}m{\colwidth}m{\colwidth}m{\colwidth}m{\colwidth}m{\colwidth}m{\colwidth}m{\colwidth}m{\colwidth}m{\colwidth}m{\colwidth}m{\colwidth}m{\colwidth}m{\colwidth}m{\colwidth}m{\colwidth}m{\colwidth}m{\colwidth}}
\textbf{Test dataset} & \multicolumn{6}{l}{{\cellcolor[rgb]{.9,.9,.9}} BNCI2014001} & \multicolumn{7}{l}{BNCI2014004} & \multicolumn{7}{l}{{\cellcolor[rgb]{.9,.9,.9}} Cho2017} & \multicolumn{6}{l}{Lee2019\_MI} & \multicolumn{5}{l}{{\cellcolor[rgb]{.9,.9,.9}} PhysionetMI(I)} & \multicolumn{7}{l}{Schirrmeister2017} & \multicolumn{7}{l}{{\cellcolor[rgb]{.9,.9,.9}} Weibo2014} & \multicolumn{6}{l}{Zhou2016} \\
\textbf{Trials/class} & {\cellcolor[rgb]{.9,.9,.9}} 1 & 2 & {\cellcolor[rgb]{.9,.9,.9}} 4 & 8 & {\cellcolor[rgb]{.9,.9,.9}} 16 & 32 & {\cellcolor[rgb]{.9,.9,.9}} 1 & 2 & {\cellcolor[rgb]{.9,.9,.9}} 4 & 8 & {\cellcolor[rgb]{.9,.9,.9}} 16 & 32 & {\cellcolor[rgb]{.9,.9,.9}} 64 & 1 & {\cellcolor[rgb]{.9,.9,.9}} 2 & 4 & {\cellcolor[rgb]{.9,.9,.9}} 8 & 16 & {\cellcolor[rgb]{.9,.9,.9}} 32 & 64 & {\cellcolor[rgb]{.9,.9,.9}} 1 & 2 & {\cellcolor[rgb]{.9,.9,.9}} 4 & 8 & {\cellcolor[rgb]{.9,.9,.9}} 16 & 32 & {\cellcolor[rgb]{.9,.9,.9}} 1 & 2 & {\cellcolor[rgb]{.9,.9,.9}} 4 & 8 & {\cellcolor[rgb]{.9,.9,.9}} 16 & 1 & {\cellcolor[rgb]{.9,.9,.9}} 2 & 4 & {\cellcolor[rgb]{.9,.9,.9}} 8 & 16 & {\cellcolor[rgb]{.9,.9,.9}} 32 & 64 & {\cellcolor[rgb]{.9,.9,.9}} 1 & 2 & {\cellcolor[rgb]{.9,.9,.9}} 4 & 8 & {\cellcolor[rgb]{.9,.9,.9}} 16 & 32 & {\cellcolor[rgb]{.9,.9,.9}} 64 & 1 & {\cellcolor[rgb]{.9,.9,.9}} 2 & 4 & {\cellcolor[rgb]{.9,.9,.9}} 8 & 16 & {\cellcolor[rgb]{.9,.9,.9}} 32 \\
\textbf{Pretraining dataset} & {\cellcolor[rgb]{.9,.9,.9}} & & {\cellcolor[rgb]{.9,.9,.9}} & & {\cellcolor[rgb]{.9,.9,.9}} & & {\cellcolor[rgb]{.9,.9,.9}} & & {\cellcolor[rgb]{.9,.9,.9}} & & {\cellcolor[rgb]{.9,.9,.9}} & & {\cellcolor[rgb]{.9,.9,.9}} & & {\cellcolor[rgb]{.9,.9,.9}} & & {\cellcolor[rgb]{.9,.9,.9}} & & {\cellcolor[rgb]{.9,.9,.9}} & & {\cellcolor[rgb]{.9,.9,.9}} & & {\cellcolor[rgb]{.9,.9,.9}} & & {\cellcolor[rgb]{.9,.9,.9}} & & {\cellcolor[rgb]{.9,.9,.9}} & & {\cellcolor[rgb]{.9,.9,.9}} & & {\cellcolor[rgb]{.9,.9,.9}} & & {\cellcolor[rgb]{.9,.9,.9}} & & {\cellcolor[rgb]{.9,.9,.9}} & & {\cellcolor[rgb]{.9,.9,.9}} & & {\cellcolor[rgb]{.9,.9,.9}} & & {\cellcolor[rgb]{.9,.9,.9}} & & {\cellcolor[rgb]{.9,.9,.9}} & & {\cellcolor[rgb]{.9,.9,.9}} & & {\cellcolor[rgb]{.9,.9,.9}} & & {\cellcolor[rgb]{.9,.9,.9}} & & {\cellcolor[rgb]{.9,.9,.9}}\\
{\cellcolor[rgb]{.9,.9,.9}} AlexMI & {\cellcolor[HTML]{F3F8FE}} \color[HTML]{000000} 51 & {\cellcolor[HTML]{EBF3FB}} \color[HTML]{000000} 53 & {\cellcolor[HTML]{E3EEF9}} \color[HTML]{000000} 55 & {\cellcolor[HTML]{DCE9F6}} \color[HTML]{000000} 57 & {\cellcolor[HTML]{CCDFF1}} \color[HTML]{000000} 61 & {\cellcolor[HTML]{BDD7EC}} \color[HTML]{000000} 64 & {\cellcolor[HTML]{E3EEF9}} \color[HTML]{000000} 55 & {\cellcolor[HTML]{DFECF7}} \color[HTML]{000000} 56 & {\cellcolor[HTML]{D3E4F3}} \color[HTML]{000000} 59 & {\cellcolor[HTML]{C8DCF0}} \color[HTML]{000000} 62 & {\cellcolor[HTML]{BDD7EC}} \color[HTML]{000000} 64 & {\cellcolor[HTML]{A9CFE5}} \color[HTML]{000000} 67 & {\cellcolor[HTML]{5DA5D1}} \color[HTML]{F1F1F1} 77 & {\cellcolor[HTML]{DCE9F6}} \color[HTML]{000000} 57 & {\cellcolor[HTML]{D8E7F5}} \color[HTML]{000000} 58 & {\cellcolor[HTML]{D3E4F3}} \color[HTML]{000000} 59 & {\cellcolor[HTML]{CCDFF1}} \color[HTML]{000000} 61 & {\cellcolor[HTML]{C8DCF0}} \color[HTML]{000000} 62 & {\cellcolor[HTML]{BDD7EC}} \color[HTML]{000000} 64 & {\cellcolor[HTML]{B0D2E7}} \color[HTML]{000000} 66 & {\cellcolor[HTML]{F3F8FE}} \color[HTML]{000000} 51 & {\cellcolor[HTML]{EFF6FC}} \color[HTML]{000000} 52 & {\cellcolor[HTML]{EBF3FB}} \color[HTML]{000000} 53 & {\cellcolor[HTML]{E3EEF9}} \color[HTML]{000000} 55 & {\cellcolor[HTML]{DFECF7}} \color[HTML]{000000} 56 & {\cellcolor[HTML]{D3E4F3}} \color[HTML]{000000} 59 & {\cellcolor[HTML]{E7F1FA}} \color[HTML]{000000} 54 & {\cellcolor[HTML]{DFECF7}} \color[HTML]{000000} 56 & {\cellcolor[HTML]{D8E7F5}} \color[HTML]{000000} 58 & {\cellcolor[HTML]{CCDFF1}} \color[HTML]{000000} 61 & {\cellcolor[HTML]{B7D4EA}} \color[HTML]{000000} 65 & {\cellcolor[HTML]{E7F1FA}} \color[HTML]{000000} 54 & {\cellcolor[HTML]{DFECF7}} \color[HTML]{000000} 56 & {\cellcolor[HTML]{D8E7F5}} \color[HTML]{000000} 58 & {\cellcolor[HTML]{D0E1F2}} \color[HTML]{000000} 60 & {\cellcolor[HTML]{BDD7EC}} \color[HTML]{000000} 64 & {\cellcolor[HTML]{B0D2E7}} \color[HTML]{000000} 66 & {\cellcolor[HTML]{9CC9E1}} \color[HTML]{000000} 69 & {\cellcolor[HTML]{F7FBFF}} \color[HTML]{000000} 48 & {\cellcolor[HTML]{F7FBFF}} \color[HTML]{000000} 50 & {\cellcolor[HTML]{F7FBFF}} \color[HTML]{000000} 50 & {\cellcolor[HTML]{F7FBFF}} \color[HTML]{000000} 50 & {\cellcolor[HTML]{F3F8FE}} \color[HTML]{000000} 51 & {\cellcolor[HTML]{EFF6FC}} \color[HTML]{000000} 52 & {\cellcolor[HTML]{DFECF7}} \color[HTML]{000000} 56 & {\cellcolor[HTML]{F3F8FE}} \color[HTML]{000000} 51 & {\cellcolor[HTML]{EFF6FC}} \color[HTML]{000000} 52 & {\cellcolor[HTML]{EFF6FC}} \color[HTML]{000000} 52 & {\cellcolor[HTML]{E7F1FA}} \color[HTML]{000000} 54 & {\cellcolor[HTML]{DFECF7}} \color[HTML]{000000} 56 & {\cellcolor[HTML]{D0E1F2}} \color[HTML]{000000} 60 \\
BNCI2014001 & {\cellcolor[HTML]{B7D4EA}} \color[HTML]{000000} 65 & {\cellcolor[HTML]{9CC9E1}} \color[HTML]{000000} 69 & {\cellcolor[HTML]{7CB7DA}} \color[HTML]{000000} 73 & \bfseries {\cellcolor[HTML]{57A0CE}} \color[HTML]{F1F1F1} 78 & \bfseries {\cellcolor[HTML]{4493C7}} \color[HTML]{F1F1F1} 81 & \bfseries {\cellcolor[HTML]{2E7EBC}} \color[HTML]{F1F1F1} 85 & {\cellcolor[HTML]{D3E4F3}} \color[HTML]{000000} 59 & {\cellcolor[HTML]{C8DCF0}} \color[HTML]{000000} 62 & {\cellcolor[HTML]{B0D2E7}} \color[HTML]{000000} 66 & {\cellcolor[HTML]{94C4DF}} \color[HTML]{000000} 70 & {\cellcolor[HTML]{6AAED6}} \color[HTML]{F1F1F1} 75 & {\cellcolor[HTML]{519CCC}} \color[HTML]{F1F1F1} 79 & {\cellcolor[HTML]{1B69AF}} \color[HTML]{F1F1F1} 89 & {\cellcolor[HTML]{D3E4F3}} \color[HTML]{000000} 59 & {\cellcolor[HTML]{CCDFF1}} \color[HTML]{000000} 61 & {\cellcolor[HTML]{C3DAEE}} \color[HTML]{000000} 63 & {\cellcolor[HTML]{BDD7EC}} \color[HTML]{000000} 64 & {\cellcolor[HTML]{B0D2E7}} \color[HTML]{000000} 66 & {\cellcolor[HTML]{A3CCE3}} \color[HTML]{000000} 68 & {\cellcolor[HTML]{9CC9E1}} \color[HTML]{000000} 69 & {\cellcolor[HTML]{DFECF7}} \color[HTML]{000000} 56 & {\cellcolor[HTML]{D3E4F3}} \color[HTML]{000000} 59 & {\cellcolor[HTML]{CCDFF1}} \color[HTML]{000000} 61 & {\cellcolor[HTML]{BDD7EC}} \color[HTML]{000000} 64 & {\cellcolor[HTML]{9CC9E1}} \color[HTML]{000000} 69 & {\cellcolor[HTML]{84BCDB}} \color[HTML]{000000} 72 & {\cellcolor[HTML]{D8E7F5}} \color[HTML]{000000} 58 & {\cellcolor[HTML]{C8DCF0}} \color[HTML]{000000} 62 & {\cellcolor[HTML]{B7D4EA}} \color[HTML]{000000} 65 & {\cellcolor[HTML]{A3CCE3}} \color[HTML]{000000} 68 & {\cellcolor[HTML]{84BCDB}} \color[HTML]{000000} 72 & {\cellcolor[HTML]{E7F1FA}} \color[HTML]{000000} 54 & {\cellcolor[HTML]{E3EEF9}} \color[HTML]{000000} 55 & {\cellcolor[HTML]{DCE9F6}} \color[HTML]{000000} 57 & {\cellcolor[HTML]{CCDFF1}} \color[HTML]{000000} 61 & {\cellcolor[HTML]{B7D4EA}} \color[HTML]{000000} 65 & {\cellcolor[HTML]{94C4DF}} \color[HTML]{000000} 70 & {\cellcolor[HTML]{7CB7DA}} \color[HTML]{000000} 73 & {\cellcolor[HTML]{EBF3FB}} \color[HTML]{000000} 53 & {\cellcolor[HTML]{E3EEF9}} \color[HTML]{000000} 55 & {\cellcolor[HTML]{DCE9F6}} \color[HTML]{000000} 57 & {\cellcolor[HTML]{D3E4F3}} \color[HTML]{000000} 59 & {\cellcolor[HTML]{BDD7EC}} \color[HTML]{000000} 64 & {\cellcolor[HTML]{8CC0DD}} \color[HTML]{000000} 71 & {\cellcolor[HTML]{74B3D8}} \color[HTML]{000000} 74 & {\cellcolor[HTML]{B0D2E7}} \color[HTML]{000000} 66 & {\cellcolor[HTML]{9CC9E1}} \color[HTML]{000000} 69 & {\cellcolor[HTML]{64A9D3}} \color[HTML]{F1F1F1} 76 & {\cellcolor[HTML]{4A98C9}} \color[HTML]{F1F1F1} 80 & {\cellcolor[HTML]{3989C1}} \color[HTML]{F1F1F1} 83 & {\cellcolor[HTML]{2979B9}} \color[HTML]{F1F1F1} 86 \\
{\cellcolor[rgb]{.9,.9,.9}} BNCI2014004 & {\cellcolor[HTML]{CCDFF1}} \color[HTML]{000000} 61 & {\cellcolor[HTML]{C8DCF0}} \color[HTML]{000000} 62 & {\cellcolor[HTML]{B7D4EA}} \color[HTML]{000000} 65 & {\cellcolor[HTML]{A3CCE3}} \color[HTML]{000000} 68 & {\cellcolor[HTML]{8CC0DD}} \color[HTML]{000000} 71 & {\cellcolor[HTML]{7CB7DA}} \color[HTML]{000000} 73 & \bfseries {\cellcolor[HTML]{6AAED6}} \color[HTML]{F1F1F1} 75 & \bfseries {\cellcolor[HTML]{519CCC}} \color[HTML]{F1F1F1} 79 & \bfseries {\cellcolor[HTML]{3E8EC4}} \color[HTML]{F1F1F1} 82 & \bfseries {\cellcolor[HTML]{2E7EBC}} \color[HTML]{F1F1F1} 85 & \bfseries {\cellcolor[HTML]{2373B6}} \color[HTML]{F1F1F1} 87 & \bfseries {\cellcolor[HTML]{1B69AF}} \color[HTML]{F1F1F1} 89 & \bfseries {\cellcolor[HTML]{084F99}} \color[HTML]{F1F1F1} 94 & {\cellcolor[HTML]{D8E7F5}} \color[HTML]{000000} 58 & {\cellcolor[HTML]{D0E1F2}} \color[HTML]{000000} 60 & {\cellcolor[HTML]{CCDFF1}} \color[HTML]{000000} 61 & {\cellcolor[HTML]{C8DCF0}} \color[HTML]{000000} 62 & {\cellcolor[HTML]{BDD7EC}} \color[HTML]{000000} 64 & {\cellcolor[HTML]{B7D4EA}} \color[HTML]{000000} 65 & {\cellcolor[HTML]{B0D2E7}} \color[HTML]{000000} 66 & {\cellcolor[HTML]{D0E1F2}} \color[HTML]{000000} 60 & {\cellcolor[HTML]{C8DCF0}} \color[HTML]{000000} 62 & {\cellcolor[HTML]{B7D4EA}} \color[HTML]{000000} 65 & {\cellcolor[HTML]{A9CFE5}} \color[HTML]{000000} 67 & {\cellcolor[HTML]{94C4DF}} \color[HTML]{000000} 70 & {\cellcolor[HTML]{7CB7DA}} \color[HTML]{000000} 73 & {\cellcolor[HTML]{DCE9F6}} \color[HTML]{000000} 57 & {\cellcolor[HTML]{D3E4F3}} \color[HTML]{000000} 59 & {\cellcolor[HTML]{D0E1F2}} \color[HTML]{000000} 60 & {\cellcolor[HTML]{C3DAEE}} \color[HTML]{000000} 63 & {\cellcolor[HTML]{B0D2E7}} \color[HTML]{000000} 66 & {\cellcolor[HTML]{DCE9F6}} \color[HTML]{000000} 57 & {\cellcolor[HTML]{D0E1F2}} \color[HTML]{000000} 60 & {\cellcolor[HTML]{C8DCF0}} \color[HTML]{000000} 62 & {\cellcolor[HTML]{B7D4EA}} \color[HTML]{000000} 65 & {\cellcolor[HTML]{A3CCE3}} \color[HTML]{000000} 68 & {\cellcolor[HTML]{8CC0DD}} \color[HTML]{000000} 71 & {\cellcolor[HTML]{74B3D8}} \color[HTML]{000000} 74 & {\cellcolor[HTML]{E3EEF9}} \color[HTML]{000000} 55 & {\cellcolor[HTML]{DCE9F6}} \color[HTML]{000000} 57 & {\cellcolor[HTML]{C8DCF0}} \color[HTML]{000000} 62 & {\cellcolor[HTML]{B7D4EA}} \color[HTML]{000000} 65 & {\cellcolor[HTML]{9CC9E1}} \color[HTML]{000000} 69 & {\cellcolor[HTML]{84BCDB}} \color[HTML]{000000} 72 & {\cellcolor[HTML]{7CB7DA}} \color[HTML]{000000} 73 & {\cellcolor[HTML]{84BCDB}} \color[HTML]{000000} 72 & {\cellcolor[HTML]{64A9D3}} \color[HTML]{F1F1F1} 76 & {\cellcolor[HTML]{4493C7}} \color[HTML]{F1F1F1} 81 & {\cellcolor[HTML]{3383BE}} \color[HTML]{F1F1F1} 84 & {\cellcolor[HTML]{2979B9}} \color[HTML]{F1F1F1} 86 & {\cellcolor[HTML]{1B69AF}} \color[HTML]{F1F1F1} 89 \\
BNCI2015001 & {\cellcolor[HTML]{D0E1F2}} \color[HTML]{000000} 60 & {\cellcolor[HTML]{C8DCF0}} \color[HTML]{000000} 62 & {\cellcolor[HTML]{B7D4EA}} \color[HTML]{000000} 65 & {\cellcolor[HTML]{A3CCE3}} \color[HTML]{000000} 68 & {\cellcolor[HTML]{84BCDB}} \color[HTML]{000000} 72 & {\cellcolor[HTML]{6AAED6}} \color[HTML]{F1F1F1} 75 & {\cellcolor[HTML]{D0E1F2}} \color[HTML]{000000} 60 & {\cellcolor[HTML]{C3DAEE}} \color[HTML]{000000} 63 & {\cellcolor[HTML]{B0D2E7}} \color[HTML]{000000} 66 & {\cellcolor[HTML]{94C4DF}} \color[HTML]{000000} 70 & {\cellcolor[HTML]{7CB7DA}} \color[HTML]{000000} 73 & {\cellcolor[HTML]{64A9D3}} \color[HTML]{F1F1F1} 76 & {\cellcolor[HTML]{2979B9}} \color[HTML]{F1F1F1} 86 & {\cellcolor[HTML]{DFECF7}} \color[HTML]{000000} 56 & {\cellcolor[HTML]{D3E4F3}} \color[HTML]{000000} 59 & {\cellcolor[HTML]{CCDFF1}} \color[HTML]{000000} 61 & {\cellcolor[HTML]{C3DAEE}} \color[HTML]{000000} 63 & {\cellcolor[HTML]{BDD7EC}} \color[HTML]{000000} 64 & {\cellcolor[HTML]{A9CFE5}} \color[HTML]{000000} 67 & {\cellcolor[HTML]{A3CCE3}} \color[HTML]{000000} 68 & {\cellcolor[HTML]{DFECF7}} \color[HTML]{000000} 56 & {\cellcolor[HTML]{D8E7F5}} \color[HTML]{000000} 58 & {\cellcolor[HTML]{D0E1F2}} \color[HTML]{000000} 60 & {\cellcolor[HTML]{C3DAEE}} \color[HTML]{000000} 63 & {\cellcolor[HTML]{B0D2E7}} \color[HTML]{000000} 66 & {\cellcolor[HTML]{9CC9E1}} \color[HTML]{000000} 69 & {\cellcolor[HTML]{E3EEF9}} \color[HTML]{000000} 55 & {\cellcolor[HTML]{DFECF7}} \color[HTML]{000000} 56 & {\cellcolor[HTML]{D3E4F3}} \color[HTML]{000000} 59 & {\cellcolor[HTML]{C8DCF0}} \color[HTML]{000000} 62 & {\cellcolor[HTML]{B0D2E7}} \color[HTML]{000000} 66 & {\cellcolor[HTML]{EBF3FB}} \color[HTML]{000000} 53 & {\cellcolor[HTML]{E7F1FA}} \color[HTML]{000000} 54 & {\cellcolor[HTML]{DFECF7}} \color[HTML]{000000} 56 & {\cellcolor[HTML]{D3E4F3}} \color[HTML]{000000} 59 & {\cellcolor[HTML]{C3DAEE}} \color[HTML]{000000} 63 & {\cellcolor[HTML]{A9CFE5}} \color[HTML]{000000} 67 & {\cellcolor[HTML]{8CC0DD}} \color[HTML]{000000} 71 & {\cellcolor[HTML]{E3EEF9}} \color[HTML]{000000} 55 & {\cellcolor[HTML]{DCE9F6}} \color[HTML]{000000} 57 & {\cellcolor[HTML]{D0E1F2}} \color[HTML]{000000} 60 & {\cellcolor[HTML]{CCDFF1}} \color[HTML]{000000} 61 & {\cellcolor[HTML]{BDD7EC}} \color[HTML]{000000} 64 & {\cellcolor[HTML]{A3CCE3}} \color[HTML]{000000} 68 & {\cellcolor[HTML]{A3CCE3}} \color[HTML]{000000} 68 & {\cellcolor[HTML]{DCE9F6}} \color[HTML]{000000} 57 & {\cellcolor[HTML]{C8DCF0}} \color[HTML]{000000} 62 & {\cellcolor[HTML]{B7D4EA}} \color[HTML]{000000} 65 & {\cellcolor[HTML]{84BCDB}} \color[HTML]{000000} 72 & {\cellcolor[HTML]{57A0CE}} \color[HTML]{F1F1F1} 78 & {\cellcolor[HTML]{3E8EC4}} \color[HTML]{F1F1F1} 82 \\
{\cellcolor[rgb]{.9,.9,.9}} BNCI2015004 & {\cellcolor[HTML]{EBF3FB}} \color[HTML]{000000} 53 & {\cellcolor[HTML]{EBF3FB}} \color[HTML]{000000} 53 & {\cellcolor[HTML]{EBF3FB}} \color[HTML]{000000} 53 & {\cellcolor[HTML]{DFECF7}} \color[HTML]{000000} 56 & {\cellcolor[HTML]{D8E7F5}} \color[HTML]{000000} 58 & {\cellcolor[HTML]{C8DCF0}} \color[HTML]{000000} 62 & {\cellcolor[HTML]{DFECF7}} \color[HTML]{000000} 56 & {\cellcolor[HTML]{D8E7F5}} \color[HTML]{000000} 58 & {\cellcolor[HTML]{D0E1F2}} \color[HTML]{000000} 60 & {\cellcolor[HTML]{C8DCF0}} \color[HTML]{000000} 62 & {\cellcolor[HTML]{B7D4EA}} \color[HTML]{000000} 65 & {\cellcolor[HTML]{A3CCE3}} \color[HTML]{000000} 68 & {\cellcolor[HTML]{57A0CE}} \color[HTML]{F1F1F1} 78 & {\cellcolor[HTML]{DFECF7}} \color[HTML]{000000} 56 & {\cellcolor[HTML]{DCE9F6}} \color[HTML]{000000} 57 & {\cellcolor[HTML]{D8E7F5}} \color[HTML]{000000} 58 & {\cellcolor[HTML]{D0E1F2}} \color[HTML]{000000} 60 & {\cellcolor[HTML]{C8DCF0}} \color[HTML]{000000} 62 & {\cellcolor[HTML]{BDD7EC}} \color[HTML]{000000} 64 & {\cellcolor[HTML]{B7D4EA}} \color[HTML]{000000} 65 & {\cellcolor[HTML]{F3F8FE}} \color[HTML]{000000} 51 & {\cellcolor[HTML]{EFF6FC}} \color[HTML]{000000} 52 & {\cellcolor[HTML]{EBF3FB}} \color[HTML]{000000} 53 & {\cellcolor[HTML]{EBF3FB}} \color[HTML]{000000} 53 & {\cellcolor[HTML]{E3EEF9}} \color[HTML]{000000} 55 & {\cellcolor[HTML]{D8E7F5}} \color[HTML]{000000} 58 & {\cellcolor[HTML]{EBF3FB}} \color[HTML]{000000} 53 & {\cellcolor[HTML]{E3EEF9}} \color[HTML]{000000} 55 & {\cellcolor[HTML]{DCE9F6}} \color[HTML]{000000} 57 & {\cellcolor[HTML]{D0E1F2}} \color[HTML]{000000} 60 & {\cellcolor[HTML]{C3DAEE}} \color[HTML]{000000} 63 & {\cellcolor[HTML]{EBF3FB}} \color[HTML]{000000} 53 & {\cellcolor[HTML]{E3EEF9}} \color[HTML]{000000} 55 & {\cellcolor[HTML]{D8E7F5}} \color[HTML]{000000} 58 & {\cellcolor[HTML]{CCDFF1}} \color[HTML]{000000} 61 & {\cellcolor[HTML]{BDD7EC}} \color[HTML]{000000} 64 & {\cellcolor[HTML]{A9CFE5}} \color[HTML]{000000} 67 & {\cellcolor[HTML]{94C4DF}} \color[HTML]{000000} 70 & {\cellcolor[HTML]{F7FBFF}} \color[HTML]{000000} 48 & {\cellcolor[HTML]{F7FBFF}} \color[HTML]{000000} 49 & {\cellcolor[HTML]{F7FBFF}} \color[HTML]{000000} 48 & {\cellcolor[HTML]{F7FBFF}} \color[HTML]{000000} 48 & {\cellcolor[HTML]{F7FBFF}} \color[HTML]{000000} 50 & {\cellcolor[HTML]{F3F8FE}} \color[HTML]{000000} 51 & {\cellcolor[HTML]{E7F1FA}} \color[HTML]{000000} 54 & {\cellcolor[HTML]{F7FBFF}} \color[HTML]{000000} 50 & {\cellcolor[HTML]{EFF6FC}} \color[HTML]{000000} 52 & {\cellcolor[HTML]{EBF3FB}} \color[HTML]{000000} 53 & {\cellcolor[HTML]{E3EEF9}} \color[HTML]{000000} 55 & {\cellcolor[HTML]{DCE9F6}} \color[HTML]{000000} 57 & {\cellcolor[HTML]{D0E1F2}} \color[HTML]{000000} 60 \\
Cho2017 & {\cellcolor[HTML]{DFECF7}} \color[HTML]{000000} 56 & {\cellcolor[HTML]{DCE9F6}} \color[HTML]{000000} 57 & {\cellcolor[HTML]{D0E1F2}} \color[HTML]{000000} 60 & {\cellcolor[HTML]{C3DAEE}} \color[HTML]{000000} 63 & {\cellcolor[HTML]{B0D2E7}} \color[HTML]{000000} 66 & {\cellcolor[HTML]{9CC9E1}} \color[HTML]{000000} 69 & {\cellcolor[HTML]{D0E1F2}} \color[HTML]{000000} 60 & {\cellcolor[HTML]{C3DAEE}} \color[HTML]{000000} 63 & {\cellcolor[HTML]{B0D2E7}} \color[HTML]{000000} 66 & {\cellcolor[HTML]{9CC9E1}} \color[HTML]{000000} 69 & {\cellcolor[HTML]{84BCDB}} \color[HTML]{000000} 72 & {\cellcolor[HTML]{7CB7DA}} \color[HTML]{000000} 73 & {\cellcolor[HTML]{4A98C9}} \color[HTML]{F1F1F1} 80 & \bfseries {\cellcolor[HTML]{C3DAEE}} \color[HTML]{000000} 63 & \bfseries {\cellcolor[HTML]{B0D2E7}} \color[HTML]{000000} 66 & \bfseries {\cellcolor[HTML]{9CC9E1}} \color[HTML]{000000} 69 & \bfseries {\cellcolor[HTML]{8CC0DD}} \color[HTML]{000000} 71 & \bfseries {\cellcolor[HTML]{74B3D8}} \color[HTML]{000000} 74 & \bfseries {\cellcolor[HTML]{64A9D3}} \color[HTML]{F1F1F1} 76 & \bfseries {\cellcolor[HTML]{57A0CE}} \color[HTML]{F1F1F1} 78 & {\cellcolor[HTML]{EBF3FB}} \color[HTML]{000000} 53 & {\cellcolor[HTML]{E3EEF9}} \color[HTML]{000000} 55 & {\cellcolor[HTML]{DCE9F6}} \color[HTML]{000000} 57 & {\cellcolor[HTML]{D8E7F5}} \color[HTML]{000000} 58 & {\cellcolor[HTML]{D0E1F2}} \color[HTML]{000000} 60 & {\cellcolor[HTML]{C8DCF0}} \color[HTML]{000000} 62 & {\cellcolor[HTML]{DFECF7}} \color[HTML]{000000} 56 & {\cellcolor[HTML]{D3E4F3}} \color[HTML]{000000} 59 & {\cellcolor[HTML]{C8DCF0}} \color[HTML]{000000} 62 & {\cellcolor[HTML]{A9CFE5}} \color[HTML]{000000} 67 & {\cellcolor[HTML]{94C4DF}} \color[HTML]{000000} 70 & {\cellcolor[HTML]{E7F1FA}} \color[HTML]{000000} 54 & {\cellcolor[HTML]{E7F1FA}} \color[HTML]{000000} 54 & {\cellcolor[HTML]{DCE9F6}} \color[HTML]{000000} 57 & {\cellcolor[HTML]{D3E4F3}} \color[HTML]{000000} 59 & {\cellcolor[HTML]{C8DCF0}} \color[HTML]{000000} 62 & {\cellcolor[HTML]{BDD7EC}} \color[HTML]{000000} 64 & {\cellcolor[HTML]{A9CFE5}} \color[HTML]{000000} 67 & {\cellcolor[HTML]{F3F8FE}} \color[HTML]{000000} 51 & {\cellcolor[HTML]{F3F8FE}} \color[HTML]{000000} 51 & {\cellcolor[HTML]{F3F8FE}} \color[HTML]{000000} 51 & {\cellcolor[HTML]{EFF6FC}} \color[HTML]{000000} 52 & {\cellcolor[HTML]{EFF6FC}} \color[HTML]{000000} 52 & {\cellcolor[HTML]{E7F1FA}} \color[HTML]{000000} 54 & {\cellcolor[HTML]{E3EEF9}} \color[HTML]{000000} 55 & {\cellcolor[HTML]{E7F1FA}} \color[HTML]{000000} 54 & {\cellcolor[HTML]{E3EEF9}} \color[HTML]{000000} 55 & {\cellcolor[HTML]{D8E7F5}} \color[HTML]{000000} 58 & {\cellcolor[HTML]{C8DCF0}} \color[HTML]{000000} 62 & {\cellcolor[HTML]{B7D4EA}} \color[HTML]{000000} 65 & {\cellcolor[HTML]{A9CFE5}} \color[HTML]{000000} 67 \\
{\cellcolor[rgb]{.9,.9,.9}} Lee2019\_MI & \bfseries {\cellcolor[HTML]{A3CCE3}} \color[HTML]{000000} 68 & \bfseries {\cellcolor[HTML]{84BCDB}} \color[HTML]{000000} 72 & \bfseries {\cellcolor[HTML]{74B3D8}} \color[HTML]{000000} 74 & {\cellcolor[HTML]{5DA5D1}} \color[HTML]{F1F1F1} 77 & {\cellcolor[HTML]{519CCC}} \color[HTML]{F1F1F1} 79 & {\cellcolor[HTML]{3E8EC4}} \color[HTML]{F1F1F1} 82 & {\cellcolor[HTML]{A3CCE3}} \color[HTML]{000000} 68 & {\cellcolor[HTML]{84BCDB}} \color[HTML]{000000} 72 & {\cellcolor[HTML]{64A9D3}} \color[HTML]{F1F1F1} 76 & {\cellcolor[HTML]{519CCC}} \color[HTML]{F1F1F1} 79 & {\cellcolor[HTML]{3E8EC4}} \color[HTML]{F1F1F1} 82 & {\cellcolor[HTML]{3383BE}} \color[HTML]{F1F1F1} 84 & {\cellcolor[HTML]{135FA7}} \color[HTML]{F1F1F1} 91 & {\cellcolor[HTML]{CCDFF1}} \color[HTML]{000000} 61 & {\cellcolor[HTML]{C3DAEE}} \color[HTML]{000000} 63 & {\cellcolor[HTML]{BDD7EC}} \color[HTML]{000000} 64 & {\cellcolor[HTML]{B0D2E7}} \color[HTML]{000000} 66 & {\cellcolor[HTML]{A3CCE3}} \color[HTML]{000000} 68 & {\cellcolor[HTML]{94C4DF}} \color[HTML]{000000} 70 & {\cellcolor[HTML]{8CC0DD}} \color[HTML]{000000} 71 & \bfseries {\cellcolor[HTML]{BDD7EC}} \color[HTML]{000000} 64 & \bfseries {\cellcolor[HTML]{A3CCE3}} \color[HTML]{000000} 68 & \bfseries {\cellcolor[HTML]{8CC0DD}} \color[HTML]{000000} 71 & \bfseries {\cellcolor[HTML]{74B3D8}} \color[HTML]{000000} 74 & \bfseries {\cellcolor[HTML]{5DA5D1}} \color[HTML]{F1F1F1} 77 & \bfseries {\cellcolor[HTML]{519CCC}} \color[HTML]{F1F1F1} 79 & \bfseries {\cellcolor[HTML]{BDD7EC}} \color[HTML]{000000} 64 & \bfseries {\cellcolor[HTML]{A9CFE5}} \color[HTML]{000000} 67 & \bfseries {\cellcolor[HTML]{94C4DF}} \color[HTML]{000000} 70 & \bfseries {\cellcolor[HTML]{7CB7DA}} \color[HTML]{000000} 73 & \bfseries {\cellcolor[HTML]{6AAED6}} \color[HTML]{F1F1F1} 75 & \bfseries {\cellcolor[HTML]{D8E7F5}} \color[HTML]{000000} 58 & \bfseries {\cellcolor[HTML]{CCDFF1}} \color[HTML]{000000} 61 & \bfseries {\cellcolor[HTML]{B7D4EA}} \color[HTML]{000000} 65 & \bfseries {\cellcolor[HTML]{A3CCE3}} \color[HTML]{000000} 68 & \bfseries {\cellcolor[HTML]{84BCDB}} \color[HTML]{000000} 72 & \bfseries {\cellcolor[HTML]{6AAED6}} \color[HTML]{F1F1F1} 75 & {\cellcolor[HTML]{5DA5D1}} \color[HTML]{F1F1F1} 77 & \bfseries {\cellcolor[HTML]{C3DAEE}} \color[HTML]{000000} 63 & \bfseries {\cellcolor[HTML]{B7D4EA}} \color[HTML]{000000} 65 & \bfseries {\cellcolor[HTML]{94C4DF}} \color[HTML]{000000} 70 & \bfseries {\cellcolor[HTML]{7CB7DA}} \color[HTML]{000000} 73 & \bfseries {\cellcolor[HTML]{5DA5D1}} \color[HTML]{F1F1F1} 77 & \bfseries {\cellcolor[HTML]{519CCC}} \color[HTML]{F1F1F1} 79 & \bfseries {\cellcolor[HTML]{519CCC}} \color[HTML]{F1F1F1} 79 & \bfseries {\cellcolor[HTML]{519CCC}} \color[HTML]{F1F1F1} 79 & {\cellcolor[HTML]{3989C1}} \color[HTML]{F1F1F1} 83 & {\cellcolor[HTML]{2373B6}} \color[HTML]{F1F1F1} 87 & {\cellcolor[HTML]{1764AB}} \color[HTML]{F1F1F1} 90 & {\cellcolor[HTML]{135FA7}} \color[HTML]{F1F1F1} 91 & \bfseries {\cellcolor[HTML]{0A549E}} \color[HTML]{F1F1F1} 93 \\
Ofner2017(I) & {\cellcolor[HTML]{F7FBFF}} \color[HTML]{000000} 50 & {\cellcolor[HTML]{F7FBFF}} \color[HTML]{000000} 50 & {\cellcolor[HTML]{F7FBFF}} \color[HTML]{000000} 50 & {\cellcolor[HTML]{F7FBFF}} \color[HTML]{000000} 50 & {\cellcolor[HTML]{F7FBFF}} \color[HTML]{000000} 50 & {\cellcolor[HTML]{F7FBFF}} \color[HTML]{000000} 50 & {\cellcolor[HTML]{F7FBFF}} \color[HTML]{000000} 50 & {\cellcolor[HTML]{F7FBFF}} \color[HTML]{000000} 50 & {\cellcolor[HTML]{F7FBFF}} \color[HTML]{000000} 50 & {\cellcolor[HTML]{F7FBFF}} \color[HTML]{000000} 50 & {\cellcolor[HTML]{F7FBFF}} \color[HTML]{000000} 50 & {\cellcolor[HTML]{F7FBFF}} \color[HTML]{000000} 50 & {\cellcolor[HTML]{F7FBFF}} \color[HTML]{000000} 50 & {\cellcolor[HTML]{F7FBFF}} \color[HTML]{000000} 50 & {\cellcolor[HTML]{F7FBFF}} \color[HTML]{000000} 50 & {\cellcolor[HTML]{F7FBFF}} \color[HTML]{000000} 50 & {\cellcolor[HTML]{F7FBFF}} \color[HTML]{000000} 50 & {\cellcolor[HTML]{E3EEF9}} \color[HTML]{000000} 55 & {\cellcolor[HTML]{D8E7F5}} \color[HTML]{000000} 58 & {\cellcolor[HTML]{D0E1F2}} \color[HTML]{000000} 60 & {\cellcolor[HTML]{F7FBFF}} \color[HTML]{000000} 50 & {\cellcolor[HTML]{F7FBFF}} \color[HTML]{000000} 50 & {\cellcolor[HTML]{F7FBFF}} \color[HTML]{000000} 50 & {\cellcolor[HTML]{F7FBFF}} \color[HTML]{000000} 50 & {\cellcolor[HTML]{F7FBFF}} \color[HTML]{000000} 50 & {\cellcolor[HTML]{F7FBFF}} \color[HTML]{000000} 50 & {\cellcolor[HTML]{F7FBFF}} \color[HTML]{000000} 50 & {\cellcolor[HTML]{F7FBFF}} \color[HTML]{000000} 50 & {\cellcolor[HTML]{F7FBFF}} \color[HTML]{000000} 50 & {\cellcolor[HTML]{F7FBFF}} \color[HTML]{000000} 50 & {\cellcolor[HTML]{F7FBFF}} \color[HTML]{000000} 50 & {\cellcolor[HTML]{F7FBFF}} \color[HTML]{000000} 50 & {\cellcolor[HTML]{F7FBFF}} \color[HTML]{000000} 50 & {\cellcolor[HTML]{F7FBFF}} \color[HTML]{000000} 50 & {\cellcolor[HTML]{F7FBFF}} \color[HTML]{000000} 50 & {\cellcolor[HTML]{F7FBFF}} \color[HTML]{000000} 50 & {\cellcolor[HTML]{F7FBFF}} \color[HTML]{000000} 50 & {\cellcolor[HTML]{F7FBFF}} \color[HTML]{000000} 50 & {\cellcolor[HTML]{F7FBFF}} \color[HTML]{000000} 50 & {\cellcolor[HTML]{F7FBFF}} \color[HTML]{000000} 50 & {\cellcolor[HTML]{F7FBFF}} \color[HTML]{000000} 50 & {\cellcolor[HTML]{F7FBFF}} \color[HTML]{000000} 50 & {\cellcolor[HTML]{F7FBFF}} \color[HTML]{000000} 50 & {\cellcolor[HTML]{F7FBFF}} \color[HTML]{000000} 50 & {\cellcolor[HTML]{F7FBFF}} \color[HTML]{000000} 50 & {\cellcolor[HTML]{F7FBFF}} \color[HTML]{000000} 50 & {\cellcolor[HTML]{F7FBFF}} \color[HTML]{000000} 50 & {\cellcolor[HTML]{F7FBFF}} \color[HTML]{000000} 50 & {\cellcolor[HTML]{F7FBFF}} \color[HTML]{000000} 50 & {\cellcolor[HTML]{F7FBFF}} \color[HTML]{000000} 50 & {\cellcolor[HTML]{F7FBFF}} \color[HTML]{000000} 50 \\
{\cellcolor[rgb]{.9,.9,.9}} PhysionetMI(I,E) & {\cellcolor[HTML]{D8E7F5}} \color[HTML]{000000} 58 & {\cellcolor[HTML]{CCDFF1}} \color[HTML]{000000} 61 & {\cellcolor[HTML]{BDD7EC}} \color[HTML]{000000} 64 & {\cellcolor[HTML]{A3CCE3}} \color[HTML]{000000} 68 & {\cellcolor[HTML]{84BCDB}} \color[HTML]{000000} 72 & {\cellcolor[HTML]{64A9D3}} \color[HTML]{F1F1F1} 76 & {\cellcolor[HTML]{DCE9F6}} \color[HTML]{000000} 57 & {\cellcolor[HTML]{D0E1F2}} \color[HTML]{000000} 60 & {\cellcolor[HTML]{C3DAEE}} \color[HTML]{000000} 63 & {\cellcolor[HTML]{A9CFE5}} \color[HTML]{000000} 67 & {\cellcolor[HTML]{94C4DF}} \color[HTML]{000000} 70 & {\cellcolor[HTML]{6AAED6}} \color[HTML]{F1F1F1} 75 & {\cellcolor[HTML]{2E7EBC}} \color[HTML]{F1F1F1} 85 & {\cellcolor[HTML]{DCE9F6}} \color[HTML]{000000} 57 & {\cellcolor[HTML]{D3E4F3}} \color[HTML]{000000} 59 & {\cellcolor[HTML]{D0E1F2}} \color[HTML]{000000} 60 & {\cellcolor[HTML]{C8DCF0}} \color[HTML]{000000} 62 & {\cellcolor[HTML]{B7D4EA}} \color[HTML]{000000} 65 & {\cellcolor[HTML]{A9CFE5}} \color[HTML]{000000} 67 & {\cellcolor[HTML]{A3CCE3}} \color[HTML]{000000} 68 & {\cellcolor[HTML]{DCE9F6}} \color[HTML]{000000} 57 & {\cellcolor[HTML]{D0E1F2}} \color[HTML]{000000} 60 & {\cellcolor[HTML]{C8DCF0}} \color[HTML]{000000} 62 & {\cellcolor[HTML]{B7D4EA}} \color[HTML]{000000} 65 & {\cellcolor[HTML]{A3CCE3}} \color[HTML]{000000} 68 & {\cellcolor[HTML]{84BCDB}} \color[HTML]{000000} 72 & {\cellcolor[HTML]{D0E1F2}} \color[HTML]{000000} 60 & {\cellcolor[HTML]{C3DAEE}} \color[HTML]{000000} 63 & {\cellcolor[HTML]{A9CFE5}} \color[HTML]{000000} 67 & {\cellcolor[HTML]{94C4DF}} \color[HTML]{000000} 70 & {\cellcolor[HTML]{74B3D8}} \color[HTML]{000000} 74 & {\cellcolor[HTML]{E7F1FA}} \color[HTML]{000000} 54 & {\cellcolor[HTML]{E3EEF9}} \color[HTML]{000000} 55 & {\cellcolor[HTML]{DCE9F6}} \color[HTML]{000000} 57 & {\cellcolor[HTML]{D0E1F2}} \color[HTML]{000000} 60 & {\cellcolor[HTML]{B7D4EA}} \color[HTML]{000000} 65 & {\cellcolor[HTML]{94C4DF}} \color[HTML]{000000} 70 & {\cellcolor[HTML]{6AAED6}} \color[HTML]{F1F1F1} 75 & {\cellcolor[HTML]{EBF3FB}} \color[HTML]{000000} 53 & {\cellcolor[HTML]{E3EEF9}} \color[HTML]{000000} 55 & {\cellcolor[HTML]{DCE9F6}} \color[HTML]{000000} 57 & {\cellcolor[HTML]{D0E1F2}} \color[HTML]{000000} 60 & {\cellcolor[HTML]{BDD7EC}} \color[HTML]{000000} 64 & {\cellcolor[HTML]{9CC9E1}} \color[HTML]{000000} 69 & {\cellcolor[HTML]{84BCDB}} \color[HTML]{000000} 72 & {\cellcolor[HTML]{CCDFF1}} \color[HTML]{000000} 61 & {\cellcolor[HTML]{B7D4EA}} \color[HTML]{000000} 65 & {\cellcolor[HTML]{94C4DF}} \color[HTML]{000000} 70 & {\cellcolor[HTML]{74B3D8}} \color[HTML]{000000} 74 & {\cellcolor[HTML]{4A98C9}} \color[HTML]{F1F1F1} 80 & {\cellcolor[HTML]{3383BE}} \color[HTML]{F1F1F1} 84 \\
Schirrmeister2017 & {\cellcolor[HTML]{D3E4F3}} \color[HTML]{000000} 59 & {\cellcolor[HTML]{C8DCF0}} \color[HTML]{000000} 62 & {\cellcolor[HTML]{B7D4EA}} \color[HTML]{000000} 65 & {\cellcolor[HTML]{9CC9E1}} \color[HTML]{000000} 69 & {\cellcolor[HTML]{74B3D8}} \color[HTML]{000000} 74 & {\cellcolor[HTML]{57A0CE}} \color[HTML]{F1F1F1} 78 & {\cellcolor[HTML]{D8E7F5}} \color[HTML]{000000} 58 & {\cellcolor[HTML]{CCDFF1}} \color[HTML]{000000} 61 & {\cellcolor[HTML]{BDD7EC}} \color[HTML]{000000} 64 & {\cellcolor[HTML]{A3CCE3}} \color[HTML]{000000} 68 & {\cellcolor[HTML]{7CB7DA}} \color[HTML]{000000} 73 & {\cellcolor[HTML]{5DA5D1}} \color[HTML]{F1F1F1} 77 & {\cellcolor[HTML]{1F6EB3}} \color[HTML]{F1F1F1} 88 & {\cellcolor[HTML]{E3EEF9}} \color[HTML]{000000} 55 & {\cellcolor[HTML]{DCE9F6}} \color[HTML]{000000} 57 & {\cellcolor[HTML]{D3E4F3}} \color[HTML]{000000} 59 & {\cellcolor[HTML]{C8DCF0}} \color[HTML]{000000} 62 & {\cellcolor[HTML]{BDD7EC}} \color[HTML]{000000} 64 & {\cellcolor[HTML]{B0D2E7}} \color[HTML]{000000} 66 & {\cellcolor[HTML]{A3CCE3}} \color[HTML]{000000} 68 & {\cellcolor[HTML]{DCE9F6}} \color[HTML]{000000} 57 & {\cellcolor[HTML]{D3E4F3}} \color[HTML]{000000} 59 & {\cellcolor[HTML]{C8DCF0}} \color[HTML]{000000} 62 & {\cellcolor[HTML]{B0D2E7}} \color[HTML]{000000} 66 & {\cellcolor[HTML]{94C4DF}} \color[HTML]{000000} 70 & {\cellcolor[HTML]{7CB7DA}} \color[HTML]{000000} 73 & {\cellcolor[HTML]{E7F1FA}} \color[HTML]{000000} 54 & {\cellcolor[HTML]{DCE9F6}} \color[HTML]{000000} 57 & {\cellcolor[HTML]{D0E1F2}} \color[HTML]{000000} 60 & {\cellcolor[HTML]{BDD7EC}} \color[HTML]{000000} 64 & {\cellcolor[HTML]{A3CCE3}} \color[HTML]{000000} 68 & {\cellcolor[HTML]{E3EEF9}} \color[HTML]{000000} 55 & {\cellcolor[HTML]{DCE9F6}} \color[HTML]{000000} 57 & {\cellcolor[HTML]{D3E4F3}} \color[HTML]{000000} 59 & {\cellcolor[HTML]{BDD7EC}} \color[HTML]{000000} 64 & {\cellcolor[HTML]{9CC9E1}} \color[HTML]{000000} 69 & {\cellcolor[HTML]{74B3D8}} \color[HTML]{000000} 74 & \bfseries {\cellcolor[HTML]{57A0CE}} \color[HTML]{F1F1F1} 78 & {\cellcolor[HTML]{E7F1FA}} \color[HTML]{000000} 54 & {\cellcolor[HTML]{E3EEF9}} \color[HTML]{000000} 55 & {\cellcolor[HTML]{D3E4F3}} \color[HTML]{000000} 59 & {\cellcolor[HTML]{C8DCF0}} \color[HTML]{000000} 62 & {\cellcolor[HTML]{B0D2E7}} \color[HTML]{000000} 66 & {\cellcolor[HTML]{94C4DF}} \color[HTML]{000000} 70 & {\cellcolor[HTML]{74B3D8}} \color[HTML]{000000} 74 & {\cellcolor[HTML]{C8DCF0}} \color[HTML]{000000} 62 & {\cellcolor[HTML]{A9CFE5}} \color[HTML]{000000} 67 & {\cellcolor[HTML]{7CB7DA}} \color[HTML]{000000} 73 & {\cellcolor[HTML]{57A0CE}} \color[HTML]{F1F1F1} 78 & {\cellcolor[HTML]{3383BE}} \color[HTML]{F1F1F1} 84 & {\cellcolor[HTML]{1F6EB3}} \color[HTML]{F1F1F1} 88 \\
{\cellcolor[rgb]{.9,.9,.9}} Weibo2014 & {\cellcolor[HTML]{DFECF7}} \color[HTML]{000000} 56 & {\cellcolor[HTML]{D8E7F5}} \color[HTML]{000000} 58 & {\cellcolor[HTML]{C8DCF0}} \color[HTML]{000000} 62 & {\cellcolor[HTML]{B7D4EA}} \color[HTML]{000000} 65 & {\cellcolor[HTML]{A3CCE3}} \color[HTML]{000000} 68 & {\cellcolor[HTML]{84BCDB}} \color[HTML]{000000} 72 & {\cellcolor[HTML]{DCE9F6}} \color[HTML]{000000} 57 & {\cellcolor[HTML]{D0E1F2}} \color[HTML]{000000} 60 & {\cellcolor[HTML]{C3DAEE}} \color[HTML]{000000} 63 & {\cellcolor[HTML]{B0D2E7}} \color[HTML]{000000} 66 & {\cellcolor[HTML]{9CC9E1}} \color[HTML]{000000} 69 & {\cellcolor[HTML]{84BCDB}} \color[HTML]{000000} 72 & {\cellcolor[HTML]{3989C1}} \color[HTML]{F1F1F1} 83 & {\cellcolor[HTML]{D3E4F3}} \color[HTML]{000000} 59 & {\cellcolor[HTML]{D0E1F2}} \color[HTML]{000000} 60 & {\cellcolor[HTML]{C8DCF0}} \color[HTML]{000000} 62 & {\cellcolor[HTML]{BDD7EC}} \color[HTML]{000000} 64 & {\cellcolor[HTML]{B7D4EA}} \color[HTML]{000000} 65 & {\cellcolor[HTML]{B0D2E7}} \color[HTML]{000000} 66 & {\cellcolor[HTML]{A9CFE5}} \color[HTML]{000000} 67 & {\cellcolor[HTML]{E3EEF9}} \color[HTML]{000000} 55 & {\cellcolor[HTML]{DCE9F6}} \color[HTML]{000000} 57 & {\cellcolor[HTML]{D8E7F5}} \color[HTML]{000000} 58 & {\cellcolor[HTML]{D0E1F2}} \color[HTML]{000000} 60 & {\cellcolor[HTML]{C3DAEE}} \color[HTML]{000000} 63 & {\cellcolor[HTML]{A9CFE5}} \color[HTML]{000000} 67 & {\cellcolor[HTML]{D3E4F3}} \color[HTML]{000000} 59 & {\cellcolor[HTML]{CCDFF1}} \color[HTML]{000000} 61 & {\cellcolor[HTML]{B7D4EA}} \color[HTML]{000000} 65 & {\cellcolor[HTML]{A3CCE3}} \color[HTML]{000000} 68 & {\cellcolor[HTML]{8CC0DD}} \color[HTML]{000000} 71 & {\cellcolor[HTML]{EBF3FB}} \color[HTML]{000000} 53 & {\cellcolor[HTML]{E3EEF9}} \color[HTML]{000000} 55 & {\cellcolor[HTML]{D8E7F5}} \color[HTML]{000000} 58 & {\cellcolor[HTML]{CCDFF1}} \color[HTML]{000000} 61 & {\cellcolor[HTML]{BDD7EC}} \color[HTML]{000000} 64 & {\cellcolor[HTML]{A3CCE3}} \color[HTML]{000000} 68 & {\cellcolor[HTML]{84BCDB}} \color[HTML]{000000} 72 & {\cellcolor[HTML]{F3F8FE}} \color[HTML]{000000} 51 & {\cellcolor[HTML]{EFF6FC}} \color[HTML]{000000} 52 & {\cellcolor[HTML]{EBF3FB}} \color[HTML]{000000} 53 & {\cellcolor[HTML]{E7F1FA}} \color[HTML]{000000} 54 & {\cellcolor[HTML]{DCE9F6}} \color[HTML]{000000} 57 & {\cellcolor[HTML]{CCDFF1}} \color[HTML]{000000} 61 & {\cellcolor[HTML]{B7D4EA}} \color[HTML]{000000} 65 & {\cellcolor[HTML]{E3EEF9}} \color[HTML]{000000} 55 & {\cellcolor[HTML]{DFECF7}} \color[HTML]{000000} 56 & {\cellcolor[HTML]{DCE9F6}} \color[HTML]{000000} 57 & {\cellcolor[HTML]{CCDFF1}} \color[HTML]{000000} 61 & {\cellcolor[HTML]{B0D2E7}} \color[HTML]{000000} 66 & {\cellcolor[HTML]{8CC0DD}} \color[HTML]{000000} 71 \\
Zhou2016 & {\cellcolor[HTML]{C3DAEE}} \color[HTML]{000000} 63 & {\cellcolor[HTML]{B7D4EA}} \color[HTML]{000000} 65 & {\cellcolor[HTML]{9CC9E1}} \color[HTML]{000000} 69 & {\cellcolor[HTML]{84BCDB}} \color[HTML]{000000} 72 & {\cellcolor[HTML]{6AAED6}} \color[HTML]{F1F1F1} 75 & {\cellcolor[HTML]{5DA5D1}} \color[HTML]{F1F1F1} 77 & {\cellcolor[HTML]{BDD7EC}} \color[HTML]{000000} 64 & {\cellcolor[HTML]{A9CFE5}} \color[HTML]{000000} 67 & {\cellcolor[HTML]{94C4DF}} \color[HTML]{000000} 70 & {\cellcolor[HTML]{74B3D8}} \color[HTML]{000000} 74 & {\cellcolor[HTML]{57A0CE}} \color[HTML]{F1F1F1} 78 & {\cellcolor[HTML]{4493C7}} \color[HTML]{F1F1F1} 81 & {\cellcolor[HTML]{1B69AF}} \color[HTML]{F1F1F1} 89 & {\cellcolor[HTML]{D0E1F2}} \color[HTML]{000000} 60 & {\cellcolor[HTML]{C8DCF0}} \color[HTML]{000000} 62 & {\cellcolor[HTML]{C3DAEE}} \color[HTML]{000000} 63 & {\cellcolor[HTML]{B7D4EA}} \color[HTML]{000000} 65 & {\cellcolor[HTML]{B0D2E7}} \color[HTML]{000000} 66 & {\cellcolor[HTML]{A3CCE3}} \color[HTML]{000000} 68 & {\cellcolor[HTML]{9CC9E1}} \color[HTML]{000000} 69 & {\cellcolor[HTML]{D0E1F2}} \color[HTML]{000000} 60 & {\cellcolor[HTML]{C3DAEE}} \color[HTML]{000000} 63 & {\cellcolor[HTML]{B0D2E7}} \color[HTML]{000000} 66 & {\cellcolor[HTML]{9CC9E1}} \color[HTML]{000000} 69 & {\cellcolor[HTML]{84BCDB}} \color[HTML]{000000} 72 & {\cellcolor[HTML]{74B3D8}} \color[HTML]{000000} 74 & {\cellcolor[HTML]{DCE9F6}} \color[HTML]{000000} 57 & {\cellcolor[HTML]{D0E1F2}} \color[HTML]{000000} 60 & {\cellcolor[HTML]{C3DAEE}} \color[HTML]{000000} 63 & {\cellcolor[HTML]{B0D2E7}} \color[HTML]{000000} 66 & {\cellcolor[HTML]{9CC9E1}} \color[HTML]{000000} 69 & {\cellcolor[HTML]{DFECF7}} \color[HTML]{000000} 56 & {\cellcolor[HTML]{D3E4F3}} \color[HTML]{000000} 59 & {\cellcolor[HTML]{C8DCF0}} \color[HTML]{000000} 62 & {\cellcolor[HTML]{B0D2E7}} \color[HTML]{000000} 66 & {\cellcolor[HTML]{94C4DF}} \color[HTML]{000000} 70 & {\cellcolor[HTML]{84BCDB}} \color[HTML]{000000} 72 & {\cellcolor[HTML]{6AAED6}} \color[HTML]{F1F1F1} 75 & {\cellcolor[HTML]{DCE9F6}} \color[HTML]{000000} 57 & {\cellcolor[HTML]{D3E4F3}} \color[HTML]{000000} 59 & {\cellcolor[HTML]{C3DAEE}} \color[HTML]{000000} 63 & {\cellcolor[HTML]{A3CCE3}} \color[HTML]{000000} 68 & {\cellcolor[HTML]{94C4DF}} \color[HTML]{000000} 70 & {\cellcolor[HTML]{7CB7DA}} \color[HTML]{000000} 73 & {\cellcolor[HTML]{6AAED6}} \color[HTML]{F1F1F1} 75 & \bfseries {\cellcolor[HTML]{519CCC}} \color[HTML]{F1F1F1} 79 & \bfseries {\cellcolor[HTML]{3383BE}} \color[HTML]{F1F1F1} 84 & \bfseries {\cellcolor[HTML]{1B69AF}} \color[HTML]{F1F1F1} 89 & \bfseries {\cellcolor[HTML]{135FA7}} \color[HTML]{F1F1F1} 91 & \bfseries {\cellcolor[HTML]{0A549E}} \color[HTML]{F1F1F1} 93 & \bfseries {\cellcolor[HTML]{0A549E}} \color[HTML]{F1F1F1} 93 \\
\end{tabular}



==> glossary.tex <==
\usepackage[acronym]{glossaries}

\makenoidxglossaries


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Glossary
\newglossaryentry{h-a-label}{
    name={human-annotated label},
    description={
    Labels that, unlike \glspl{pseudo-label}, were manually annotated by humans or, 
    in the context of \acrshort{bci}, that required the subject to execute a pre-scripted task.
    Examples of such labels in \acrshort{bci} are the imagery class that was executed during an epoch, the stimulus that was attended during an epoch, the sleep phase, the reported mental workload, the level of drowsiness, etc.
    However, we would not consider the subject's id or the electrode names as human-annotated labels
    },
}

\newglossaryentry{pseudo-label}{
    name={pseudo label},
    description={
        Pseudo labels, unlike \glspl{h-a-label}, are automatically generated labels based on data attributes (e.g., chronological order of the time samples, spatial position of the electrodes),
        or on the meta-data associated with the recordings, (i.g., subject id, subject age, electrode names, etc.)
    },
}

\newglossaryentry{unsupervised-learning}
{
    name={unsupervised learning},
    description={Machine learning algorithms that do not use \glspl{h-a-label}
    },
}

\newglossaryentry{pretext-task}{
    name={pretext task},
    description={
        Learning task on which a network can be pre-trained. Training for pretext tasks is typically done by \gls{unsupervised-learning} algorithms
    },
}

\newglossaryentry{downstream-task}{
    name={downstream task},
    description={
        Learning task on which a network can be pre-trained. Downstream tasks are typically supervised.
        In the context of BCI, downstream tasks can be the classification of imagined concepts, responses to sensory stimuli, sleep stages, emotions, mental workload, drowsiness, seizure, etc  
    },
}

\newglossaryentry{sslg}
{
    name={self-supervised learning},
    description={Subset of the \gls{unsupervised-learning} algorithms that are trained with \glspl{pseudo-label}~\cite{jingSelfSupervisedVisualFeature2021}
    }
}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Acronyms

\newacronym{eeg}{EEG}{Electroencephalogram}
\newacronym{bci}{BCI}{Brain-Computer Interface}
\newacronym{dl}{DL}{Deep Learning}
\newacronym[see={[Glossary:]{sslg}}]{ssl}{SSL}{Self-Supervised Learning}
\newacronym{gan}{GAN}{Generative Adversarial Networks}
\newacronym{pca}{PCA}{Principal Component Analysis}
\newacronym{umap}{UMAP}{Uniform Manifold Approximation and Projection}
\newacronym{tsne}{t-SNE}{t-distributed Stochastic Neighbor Embedding}
\newacronym{fft}{FFT}{Fast Fourier Transform}
\newacronym{fitsne}{FIt-SNE}{\gls{fft}-accelerated interpolation-based \gls{tsne}}
\newacronym{svm}{SVM}{Support Vector Machine}
\newacronym{sae}{SAE}{Sparse Autoencoder}
\newacronym{mae}{MAE}{Masked Autoencoder}
\newacronym{dae}{DAE}{Denoising Autoencoder}
\newacronym{vae}{VAE}{Variational Autoencoder}
\newacronym{cnn}{CNN}{Convolutional Neural Network}
\newacronym{dnn}{DNN}{Deep Neural Network}
\newacronym{mlp}{MLP}{Multilayer Perceptron}
\newacronym{ica}{ICA}{Independent Component Analysis}


